InfiBench: Evaluating the Question-Answering Capabilities of Code Large Language Models

Large Language Models for code (code LLMs) have witnessed tremendous progress in recent years. With the rapid development of code LLMs, many popular evaluation benchmarks, such as HumanEval, DS-1000, and MBPP, have emerged to measure the performance of code LLMs with a particular focus on code generation tasks. However, they are insufficient to cover the full range of expected capabilities of code LLMs, which span beyond code generation to answering diverse coding-related questions. To fill this gap, we propose InfiBench, the first large-scale freeform question-answering (QA) benchmark for code to our knowledge, comprising 234 carefully selected high-quality Stack Overflow questions that span across 15 programming languages. InfiBench uses four types of model-free automatic metrics to evaluate response correctness where domain experts carefully concretize the criterion for each question. We conduct a systematic evaluation for over 100 latest code LLMs on InfiBench, leading to a series of novel and insightful findings. Our detailed analyses showcase potential directions for further advancement of code LLMs. InfiBench is fully open source at https://infi-coder.github.io/infibench and continuously expanding to foster more scientific and systematic practices for code LLM evaluation.

==> contents/pure_abs.tex <==

\begin{abstract}
Large Language Models for understanding and generating code (code LLMs) have witnessed tremendous progress in recent years. With the rapid development of code LLMs, many popular evaluation benchmarks, such as HumanEval, DS-1000, and MBPP, have emerged to measure the performance of code LLMs with a particular focus on code generation tasks. However, they are insufficient to cover the full range of expected capabilities of code LLMs, which span beyond code generation to answering diverse coding-related questions. To fill this gap, we propose InfiCoder-Eval, a large-scale freeform question-answering (QA) benchmark for code, comprising 234 carefully selected high-quality Stack Overflow questions that span across 15 programming languages. To evaluate the response correctness, InfiCoder-Eval supports four types of model-free metrics and domain experts carefully choose and concretize the criterion for each question. We conduct a systematic evaluation for more than 80 code LLMs on InfiCoder-Eval, leading to a series of insightful findings. Furthermore, our detailed analyses showcase possible directions for further improvement of code LLMs. InfiCoder-Eval will be fully open source and continuously maintained and expanded to foster more scientific and systematic practices for evaluating code LLMs.
\end{abstract}

==> tables/main_table.tex <==
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Model} & \# Params. & \sysname & HumanEval \\
& (in B) & Score & pass@1 \\
\midrule
GPT-4 & \multirow{2}{*}{/} & \multirow{2}{*}{\witherr{$59.13\%$}{$0.58\%$}} & \multirow{2}{*}{$88.4\%$} \\ 
\cite{OpenAI2023GPT4TR} \\

deepseek-coder-33b-instruct & \multirow{2}{*}{33} & \multirow{2}{*}{$50.34\%$} & \multirow{2}{*}{$79.3\%$} \\ 
\cite{deepseekcoder} \\

GPT-3.5 & \multirow{2}{*}{/} & \multirow{2}{*}{\witherr{$46.84\%$}{$0.70\%$}} & \multirow{2}{*}{$73.2\%$} \\ 
\cite{openai_models} \\

WizardCoder-Python-34B & \multirow{2}{*}{34} & \multirow{2}{*}{$45.16\%$} & \multirow{2}{*}{$73.2\%$} \\ 
\cite{luo2023wizardcoder} \\

CodeLlama-34B-Instruct & \multirow{2}{*}{34} & \multirow{2}{*}{$43.71\%$} & \multirow{2}{*}{$41.5\%$} \\ 
\cite{roziere2023code} \\

% deepseek-coder-6.7b-instruct & 6.7 & \witherr{$42.97\%$}{$0.22\%$} &  \\ 
% WizardCoder-Python-13B & 13 & \witherr{$41.22\%$}{$0.75\%$} &  \\ 
% WizardCoder-Python-7B & 7 & \witherr{$40.30\%$}{$1.15\%$} &  \\ 
% CodeLlama-34B & 34 & $39.75\%$ & \\ 
Zypher-7b-$\beta$ & \multirow{2}{*}{7} & \multirow{2}{*}{\witherr{$39.59\%$}{$0.68\%$}} & \multirow{2}{*}{$32.38\%$} \\ 
\cite{tunstall2023zephyr} \\

OctoCoder & \multirow{2}{*}{15.5} & \multirow{2}{*}{\witherr{$37.72\%$}{$0.58\%$}} & \multirow{2}{*}{$46.2\%$} \\ 
\cite{muennighoff2023octopack} \\

% CodeLlama-13B-Instruct & 13 & \witherr{$37.18\%$}{$0.51\%$} &  \\ 
Qwen-14B-Chat & \multirow{2}{*}{14} & \multirow{2}{*}{\witherr{$36.93\%$}{$0.12\%$}} & \multirow{2}{*}{$43.9\%$} \\ 
\cite{bai2023qwen} \\

% CodeLlama-13B & 13 & \witherr{$33.92\%$}{$0.64\%$} &  \\ 
% WizardCoder-15B & 15 & \witherr{$33.34\%$}{$0.74\%$} &  \\ 
% CodeLlama-34B-Python & 34 & $33.23\%$ & \\ 
% OctoGeeX & 6 & \witherr{$32.60\%$}{$1.02\%$} &  \\ 
% Qwen-7B-Chat & 7 & \witherr{$32.48\%$}{$0.71\%$} &  \\ 
% CodeLlama-13B-Python & 13 & \witherr{$32.43\%$}{$0.42\%$} &  \\ 
% CodeLlama-7B & 7 & \witherr{$31.07\%$}{$0.87\%$} &  \\ 
% WizardCoder-3B & 3 & \witherr{$30.94\%$}{$0.60\%$} &  \\ 
Baichuan2-13B-Chat & \multirow{2}{*}{13} & \multirow{2}{*}{\witherr{$30.34\%$}{$0.76\%$}} & \multirow{2}{*}{$17.07\%$\tablefootnote{This is the score of the base model. Chat model number not reported yet.}}  \\ 
\cite{yang2023baichuan} \\

% CodeLlama-7B-Instruct & 7 & \witherr{$29.51\%$}{$0.97\%$} &  \\ 
% CodeLlama-7B-Python & 7 & \witherr{$28.88\%$}{$0.45\%$} &  \\ 
% WizardCoder-1B & 1 & \witherr{$27.11\%$}{$0.85\%$} &  \\ 
StarCoder & \multirow{2}{*}{15.5} & \multirow{2}{*}{\witherr{$26.79\%$}{$0.18\%$}} & \multirow{2}{*}{$33.6\%$} \\ 
\cite{li2023starcoder} \\
% StarCoderPlus & 15.5 & \witherr{$26.07\%$}{$1.25\%$} &  \\ 
CodeGen2.5-7B-instruct & \multirow{2}{*}{7} & \multirow{2}{*}{\witherr{$25.67\%$}{$1.57\%$}} & \multirow{2}{*}{$36.20\%$} \\ 
\cite{nijkamp2023codegen2} \\
% Baichuan2-7B-Chat & 7 & \witherr{$24.39\%$}{$0.25\%$} &  \\ 
davinci-002 & \multirow{2}{*}{/} & \multirow{2}{*}{\witherr{$19.08\%$}{$1.00\%$}} & \multirow{2}{*}{$47.0\%$\tablefootnote{This is the score of code-davinci-002. Score of davinci-002 base model not reported yet.}} \\ 
\cite{openai_models} \\
phi-1.5 & \multirow{2}{*}{1.5} & \multirow{2}{*}{\witherr{$16.63\%$}{$0.03\%$}} & \multirow{2}{*}{$34.1\%$} \\ 
\cite{li2023textbooks} \\
CodeGeeX2 & \multirow{2}{*}{6} & \multirow{2}{*}{\witherr{$16.50\%$}{$0.39\%$}} & \multirow{2}{*}{$35.9\%$} \\ 
\cite{zheng2023codegeex} \\
% phi-1 & 1.3 & \witherr{$12.84\%$}{$0.73\%$} &  \\ 
\bottomrule
\end{tabular}

==> tables/score_breakdown.tex <==

% \begin{table*}
%     \caption{Scores of all benchmarked LLMs by difficulty levels, problem types, and evaluation metrics.}
%     \label{tab:score-breakdown}
%     \centering
%     \resizebox{0.97\linewidth}{!}{
    
%     \begin{tabular}{cll|c|ccccc|cccc|cccc}
%         \toprule
%         & & & Overall & \multicolumn{5}{c|}{Difficulty Levels} & \multicolumn{4}{c|}{Problem Types} & \multicolumn{4}{c}{Evaluation Metrics} \\

        
%         \cline{4-17}

%         No & Family & Model Name & \sysname & & & & & & Code & Code & Knowledge & Config \& Env & Keyword & Unit & Blank & Text \\

%          &  & & Score & Level 1 & Level 2 & Level 3 & Level 4 & Level 5 & Completion & Debugging & QA & Debugging & Matching & Testing & Filling & Similarity \\

%         \hline\hline

%  \multicolumn{3}{c|}{max}                             & \colorbox[rgb]{0.4297,0.8573,0.3074}{70.64\%} & \colorbox[rgb]{0.2486,0.8120,0.0874}{93.08\%} & \colorbox[rgb]{0.2534,0.8132,0.0933}{92.48\%} & \colorbox[rgb]{0.5628,0.8906,0.4690}{54.16\%} & \colorbox[rgb]{0.7424,0.9355,0.6872}{31.91\%} & \colorbox[rgb]{0.8599,0.9649,0.8298}{17.36\%} & \colorbox[rgb]{0.3927,0.8480,0.2624}{75.23\%} & \colorbox[rgb]{0.4370,0.8591,0.3163}{69.74\%} & \colorbox[rgb]{0.4466,0.8615,0.3279}{68.55\%} & \colorbox[rgb]{0.4621,0.8654,0.3468}{66.63\%} & \colorbox[rgb]{0.4623,0.8654,0.3470}{66.61\%} & \colorbox[rgb]{0.3784,0.8445,0.2451}{77.00\%} & \colorbox[rgb]{0.5311,0.8827,0.4306}{58.08\%} & \colorbox[rgb]{0.3197,0.8298,0.1738}{84.27\%} \\
%  \multicolumn{3}{c|}{mean}                            & \colorbox[rgb]{0.7031,0.9257,0.6394}{36.78\%} & \colorbox[rgb]{0.5489,0.8871,0.4522}{55.88\%} & \colorbox[rgb]{0.7023,0.9255,0.6385}{36.87\%} & \colorbox[rgb]{0.8037,0.9509,0.7616}{24.32\%} & \colorbox[rgb]{0.9200,0.9800,0.9028}{9.91\%} & \colorbox[rgb]{0.9556,0.9889,0.9461}{5.50\%} & \colorbox[rgb]{0.6952,0.9237,0.6298}{37.76\%} & \colorbox[rgb]{0.7141,0.9285,0.6528}{35.41\%} & \colorbox[rgb]{0.6708,0.9176,0.6002}{40.78\%} & \colorbox[rgb]{0.7429,0.9357,0.6877}{31.85\%} & \colorbox[rgb]{0.6997,0.9249,0.6353}{37.20\%} & \colorbox[rgb]{0.7070,0.9267,0.6441}{36.30\%} & \colorbox[rgb]{0.8459,0.9614,0.8128}{19.09\%} & \colorbox[rgb]{0.8161,0.9540,0.7767}{22.78\%} \\
%  \multicolumn{3}{c|}{min}                            & \colorbox[rgb]{0.9412,0.9853,0.9286}{7.28\%} & \colorbox[rgb]{0.9265,0.9816,0.9107}{9.11\%} & \colorbox[rgb]{0.9373,0.9843,0.9238}{7.77\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.9920,0.9980,0.9903}{0.99\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.9676,0.9919,0.9607}{4.01\%} & \colorbox[rgb]{0.9331,0.9833,0.9187}{8.29\%} & \colorbox[rgb]{0.9458,0.9864,0.9342}{6.71\%} & \colorbox[rgb]{0.9616,0.9904,0.9533}{4.76\%} & \colorbox[rgb]{0.9321,0.9830,0.9175}{8.41\%} & \colorbox[rgb]{0.9731,0.9933,0.9674}{3.33\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
%  \hline
%  1 & GPT4                           & GPT4-0613                      & \colorbox[rgb]{0.4297,0.8573,0.3074}{70.64\%} & \colorbox[rgb]{0.2548,0.8135,0.0950}{92.31\%} & \colorbox[rgb]{0.2534,0.8132,0.0933}{92.48\%} & \colorbox[rgb]{0.5810,0.8952,0.4912}{51.90\%} & \colorbox[rgb]{0.7424,0.9355,0.6872}{31.91\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.3927,0.8480,0.2624}{75.23\%} & \colorbox[rgb]{0.4370,0.8591,0.3163}{69.74\%} & \colorbox[rgb]{0.4466,0.8615,0.3279}{68.55\%} & \colorbox[rgb]{0.4621,0.8654,0.3468}{66.63\%} & \colorbox[rgb]{0.4623,0.8654,0.3470}{66.61\%} & \colorbox[rgb]{0.3865,0.8465,0.2549}{76.00\%} & \colorbox[rgb]{0.5311,0.8827,0.4306}{58.08\%} & \colorbox[rgb]{0.3197,0.8298,0.1738}{84.27\%} \\
%  2 & GPT4                           & GPT4-turbo-1106                & \colorbox[rgb]{0.4476,0.8618,0.3292}{68.42\%} & \colorbox[rgb]{0.2742,0.8184,0.1186}{89.90\%} & \colorbox[rgb]{0.3657,0.8413,0.2297}{78.57\%} & \colorbox[rgb]{0.5628,0.8906,0.4690}{54.16\%} & \colorbox[rgb]{0.7503,0.9375,0.6968}{30.93\%} & \colorbox[rgb]{0.8692,0.9673,0.8412}{16.20\%} & \colorbox[rgb]{0.3960,0.8489,0.2665}{74.82\%} & \colorbox[rgb]{0.4723,0.8680,0.3592}{65.36\%} & \colorbox[rgb]{0.4553,0.8637,0.3385}{67.47\%} & \colorbox[rgb]{0.4916,0.8728,0.3825}{62.98\%} & \colorbox[rgb]{0.4754,0.8687,0.3629}{64.98\%} & \colorbox[rgb]{0.3832,0.8457,0.2510}{76.40\%} & \colorbox[rgb]{0.5648,0.8911,0.4715}{53.91\%} & \colorbox[rgb]{0.5733,0.8932,0.4819}{52.85\%} \\
%  3 & DeepSeek Coder                 & deepseek-coder-33b-instruct    & \colorbox[rgb]{0.4917,0.8728,0.3827}{62.96\%} & \colorbox[rgb]{0.2930,0.8231,0.1414}{87.58\%} & \colorbox[rgb]{0.4186,0.8545,0.2939}{72.02\%} & \colorbox[rgb]{0.6438,0.9109,0.5674}{44.12\%} & \colorbox[rgb]{0.8722,0.9680,0.8448}{15.83\%} & \colorbox[rgb]{0.8654,0.9663,0.8366}{16.67\%} & \colorbox[rgb]{0.4247,0.8561,0.3014}{71.26\%} & \colorbox[rgb]{0.5387,0.8846,0.4398}{57.14\%} & \colorbox[rgb]{0.4903,0.8725,0.3810}{63.14\%} & \colorbox[rgb]{0.5414,0.8852,0.4430}{56.81\%} & \colorbox[rgb]{0.5236,0.8808,0.4215}{59.01\%} & \colorbox[rgb]{0.3784,0.8445,0.2451}{77.00\%} & \colorbox[rgb]{0.7578,0.9394,0.7059}{30.00\%} & \colorbox[rgb]{0.7086,0.9271,0.6462}{36.09\%} \\
%  4 & Phind                          & Phind-CodeLlama-34B-v2         & \colorbox[rgb]{0.5237,0.8808,0.4216}{59.00\%} & \colorbox[rgb]{0.3245,0.8310,0.1797}{83.67\%} & \colorbox[rgb]{0.5514,0.8877,0.4552}{55.57\%} & \colorbox[rgb]{0.5712,0.8927,0.4792}{53.12\%} & \colorbox[rgb]{0.8782,0.9695,0.8521}{15.09\%} & \colorbox[rgb]{0.8795,0.9698,0.8536}{14.93\%} & \colorbox[rgb]{0.5298,0.8824,0.4290}{58.24\%} & \colorbox[rgb]{0.5293,0.8822,0.4284}{58.30\%} & \colorbox[rgb]{0.4866,0.8715,0.3765}{63.60\%} & \colorbox[rgb]{0.5533,0.8882,0.4575}{55.33\%} & \colorbox[rgb]{0.5186,0.8795,0.4154}{59.63\%} & \colorbox[rgb]{0.5285,0.8820,0.4274}{58.40\%} & \colorbox[rgb]{0.7153,0.9288,0.6543}{35.26\%} & \colorbox[rgb]{0.8047,0.9511,0.7628}{24.19\%} \\
%  5 & Phind                          & Phind-CodeLlama-34B-v1         & \colorbox[rgb]{0.5280,0.8819,0.4268}{58.47\%} & \colorbox[rgb]{0.3430,0.8356,0.2022}{81.38\%} & \colorbox[rgb]{0.4845,0.8710,0.3740}{63.85\%} & \colorbox[rgb]{0.6202,0.9050,0.5387}{47.05\%} & \colorbox[rgb]{0.8173,0.9543,0.7781}{22.63\%} & \colorbox[rgb]{0.9579,0.9895,0.9489}{5.21\%} & \colorbox[rgb]{0.4661,0.8664,0.3517}{66.13\%} & \colorbox[rgb]{0.5403,0.8850,0.4418}{56.94\%} & \colorbox[rgb]{0.5415,0.8853,0.4432}{56.79\%} & \colorbox[rgb]{0.6005,0.9001,0.5149}{49.48\%} & \colorbox[rgb]{0.5503,0.8875,0.4538}{55.71\%} & \colorbox[rgb]{0.4672,0.8667,0.3529}{66.00\%} & \colorbox[rgb]{0.6869,0.9217,0.6198}{38.78\%} & \colorbox[rgb]{0.7143,0.9285,0.6530}{35.39\%} \\
%  6 & DeepSeek LLM                   & deepseek-llm-67b-chat          & \colorbox[rgb]{0.5365,0.8840,0.4372}{57.41\%} & \colorbox[rgb]{0.3303,0.8324,0.1867}{82.96\%} & \colorbox[rgb]{0.4912,0.8727,0.3821}{63.03\%} & \colorbox[rgb]{0.6844,0.9210,0.6168}{39.09\%} & \colorbox[rgb]{0.8176,0.9543,0.7784}{22.60\%} & \colorbox[rgb]{0.9579,0.9895,0.9489}{5.21\%} & \colorbox[rgb]{0.5042,0.8759,0.3978}{61.42\%} & \colorbox[rgb]{0.5743,0.8935,0.4830}{52.73\%} & \colorbox[rgb]{0.5260,0.8814,0.4243}{58.72\%} & \colorbox[rgb]{0.5509,0.8876,0.4546}{55.63\%} & \colorbox[rgb]{0.5710,0.8927,0.4790}{53.14\%} & \colorbox[rgb]{0.4914,0.8727,0.3823}{63.00\%} & \colorbox[rgb]{0.5850,0.8962,0.4960}{51.41\%} & \colorbox[rgb]{0.7039,0.9259,0.6404}{36.68\%} \\
%  7 & GPT3.5                         & GPT-3.5-turbo-0613             & \colorbox[rgb]{0.5441,0.8859,0.4464}{56.47\%} & \colorbox[rgb]{0.2486,0.8120,0.0874}{93.08\%} & \colorbox[rgb]{0.5982,0.8995,0.5121}{49.77\%} & \colorbox[rgb]{0.7468,0.9367,0.6925}{31.36\%} & \colorbox[rgb]{0.8846,0.9711,0.8598}{14.30\%} & \colorbox[rgb]{0.9383,0.9846,0.9251}{7.64\%} & \colorbox[rgb]{0.4760,0.8689,0.3636}{64.91\%} & \colorbox[rgb]{0.6085,0.9020,0.5245}{48.50\%} & \colorbox[rgb]{0.5199,0.8799,0.4170}{59.47\%} & \colorbox[rgb]{0.5993,0.8997,0.5133}{49.64\%} & \colorbox[rgb]{0.5860,0.8964,0.4973}{51.28\%} & \colorbox[rgb]{0.4343,0.8585,0.3130}{70.07\%} & \colorbox[rgb]{0.6698,0.9174,0.5990}{40.90\%} & \colorbox[rgb]{0.6760,0.9189,0.6066}{40.13\%} \\
%  8 & Mixtral                        & mixtral-8x7B-Instruct          & \colorbox[rgb]{0.5515,0.8878,0.4554}{55.55\%} & \colorbox[rgb]{0.3365,0.8340,0.1942}{82.19\%} & \colorbox[rgb]{0.5421,0.8854,0.4439}{56.72\%} & \colorbox[rgb]{0.7455,0.9363,0.6909}{31.53\%} & \colorbox[rgb]{0.8062,0.9515,0.7647}{24.00\%} & \colorbox[rgb]{0.8599,0.9649,0.8298}{17.36\%} & \colorbox[rgb]{0.5640,0.8909,0.4705}{54.01\%} & \colorbox[rgb]{0.5837,0.8958,0.4944}{51.57\%} & \colorbox[rgb]{0.4858,0.8713,0.3756}{63.69\%} & \colorbox[rgb]{0.5674,0.8917,0.4746}{53.59\%} & \colorbox[rgb]{0.5468,0.8866,0.4496}{56.14\%} & \colorbox[rgb]{0.5931,0.8982,0.5059}{50.40\%} & \colorbox[rgb]{0.7128,0.9281,0.6512}{35.58\%} & \colorbox[rgb]{0.5015,0.8753,0.3946}{61.75\%} \\
%  9 & Qwen                           & Qwen-72B                       & \colorbox[rgb]{0.5532,0.8882,0.4574}{55.34\%} & \colorbox[rgb]{0.3382,0.8344,0.1963}{81.98\%} & \colorbox[rgb]{0.5366,0.8841,0.4373}{57.40\%} & \colorbox[rgb]{0.6641,0.9159,0.5921}{41.61\%} & \colorbox[rgb]{0.8931,0.9733,0.8702}{13.24\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.5071,0.8767,0.4014}{61.06\%} & \colorbox[rgb]{0.5708,0.8926,0.4788}{53.16\%} & \colorbox[rgb]{0.5254,0.8812,0.4236}{58.79\%} & \colorbox[rgb]{0.6445,0.9111,0.5683}{44.03\%} & \colorbox[rgb]{0.5929,0.8981,0.5056}{50.43\%} & \colorbox[rgb]{0.4833,0.8707,0.3725}{64.00\%} & \colorbox[rgb]{0.6290,0.9072,0.5494}{45.96\%} & \colorbox[rgb]{0.7061,0.9265,0.6430}{36.41\%} \\
% 10 & DeepSeek Coder                 & deepseek-coder-6.7b-instruct   & \colorbox[rgb]{0.5701,0.8924,0.4779}{53.25\%} & \colorbox[rgb]{0.3713,0.8427,0.2365}{77.88\%} & \colorbox[rgb]{0.5455,0.8863,0.4480}{56.30\%} & \colorbox[rgb]{0.7160,0.9289,0.6551}{35.18\%} & \colorbox[rgb]{0.8475,0.9618,0.8148}{18.89\%} & \colorbox[rgb]{0.9215,0.9804,0.9047}{9.72\%} & \colorbox[rgb]{0.4676,0.8668,0.3534}{65.95\%} & \colorbox[rgb]{0.6251,0.9062,0.5447}{46.44\%} & \colorbox[rgb]{0.5765,0.8940,0.4857}{52.46\%} & \colorbox[rgb]{0.6600,0.9149,0.5871}{42.12\%} & \colorbox[rgb]{0.6106,0.9026,0.5271}{48.24\%} & \colorbox[rgb]{0.4317,0.8578,0.3098}{70.40\%} & \colorbox[rgb]{0.7828,0.9457,0.7363}{26.90\%} & \colorbox[rgb]{0.8104,0.9526,0.7698}{23.48\%} \\
% 11 & Qwen                           & Qwen-72B-Chat                  & \colorbox[rgb]{0.5724,0.8930,0.4807}{52.97\%} & \colorbox[rgb]{0.3345,0.8335,0.1918}{82.44\%} & \colorbox[rgb]{0.6206,0.9051,0.5392}{47.00\%} & \colorbox[rgb]{0.7086,0.9271,0.6462}{36.09\%} & \colorbox[rgb]{0.8519,0.9630,0.8202}{18.34\%} & \colorbox[rgb]{0.9243,0.9811,0.9080}{9.38\%} & \colorbox[rgb]{0.5264,0.8815,0.4248}{58.67\%} & \colorbox[rgb]{0.6302,0.9075,0.5509}{45.81\%} & \colorbox[rgb]{0.5147,0.8786,0.4106}{60.12\%} & \colorbox[rgb]{0.6423,0.9105,0.5656}{44.31\%} & \colorbox[rgb]{0.6023,0.9005,0.5171}{49.26\%} & \colorbox[rgb]{0.5237,0.8808,0.4216}{59.00\%} & \colorbox[rgb]{0.6522,0.9130,0.5776}{43.08\%} & \colorbox[rgb]{0.7259,0.9314,0.6672}{33.95\%} \\
% 12 & Magicoder                      & Magicoder-S-CL-7B              & \colorbox[rgb]{0.5745,0.8935,0.4832}{52.71\%} & \colorbox[rgb]{0.3705,0.8425,0.2356}{77.97\%} & \colorbox[rgb]{0.5930,0.8982,0.5057}{50.42\%} & \colorbox[rgb]{0.6755,0.9188,0.6059}{40.20\%} & \colorbox[rgb]{0.8914,0.9728,0.8681}{13.45\%} & \colorbox[rgb]{0.8991,0.9748,0.8774}{12.50\%} & \colorbox[rgb]{0.5851,0.8962,0.4962}{51.39\%} & \colorbox[rgb]{0.5804,0.8950,0.4904}{51.98\%} & \colorbox[rgb]{0.5401,0.8849,0.4415}{56.97\%} & \colorbox[rgb]{0.5917,0.8978,0.5041}{50.58\%} & \colorbox[rgb]{0.5699,0.8924,0.4776}{53.28\%} & \colorbox[rgb]{0.5425,0.8855,0.4444}{56.67\%} & \colorbox[rgb]{0.8272,0.9568,0.7901}{21.41\%} & \colorbox[rgb]{0.7823,0.9455,0.7356}{26.97\%} \\
% 13 & WizardLM                       & WizardCoder-Python-34B-V1.0    & \colorbox[rgb]{0.5754,0.8938,0.4844}{52.59\%} & \colorbox[rgb]{0.3662,0.8414,0.2303}{78.51\%} & \colorbox[rgb]{0.5762,0.8940,0.4853}{52.50\%} & \colorbox[rgb]{0.7235,0.9308,0.6642}{34.25\%} & \colorbox[rgb]{0.8381,0.9595,0.8034}{20.05\%} & \colorbox[rgb]{0.9159,0.9790,0.8978}{10.42\%} & \colorbox[rgb]{0.5130,0.8782,0.4086}{60.32\%} & \colorbox[rgb]{0.6255,0.9063,0.5452}{46.39\%} & \colorbox[rgb]{0.5490,0.8872,0.4523}{55.86\%} & \colorbox[rgb]{0.6447,0.9111,0.5685}{44.01\%} & \colorbox[rgb]{0.6066,0.9016,0.5223}{48.73\%} & \colorbox[rgb]{0.4833,0.8707,0.3725}{64.00\%} & \colorbox[rgb]{0.6968,0.9241,0.6318}{37.56\%} & \colorbox[rgb]{0.8004,0.9501,0.7576}{24.72\%} \\
% 14 & Phind                          & Phind-CodeLlama-34B-Python-v1  & \colorbox[rgb]{0.5788,0.8946,0.4885}{52.17\%} & \colorbox[rgb]{0.3498,0.8373,0.2104}{80.54\%} & \colorbox[rgb]{0.6089,0.9022,0.5251}{48.44\%} & \colorbox[rgb]{0.6563,0.9140,0.5825}{42.58\%} & \colorbox[rgb]{0.9308,0.9827,0.9160}{8.57\%} & \colorbox[rgb]{0.9916,0.9979,0.9898}{1.04\%} & \colorbox[rgb]{0.5607,0.8901,0.4666}{54.41\%} & \colorbox[rgb]{0.5775,0.8943,0.4869}{52.34\%} & \colorbox[rgb]{0.5390,0.8846,0.4401}{57.11\%} & \colorbox[rgb]{0.6652,0.9162,0.5934}{41.47\%} & \colorbox[rgb]{0.5880,0.8969,0.4996}{51.04\%} & \colorbox[rgb]{0.5334,0.8832,0.4333}{57.80\%} & \colorbox[rgb]{0.7806,0.9451,0.7335}{27.18\%} & \colorbox[rgb]{0.6790,0.9197,0.6102}{39.76\%} \\
% 15 & Magicoder                      & Magicoder-S-DS-6.7B            & \colorbox[rgb]{0.5846,0.8961,0.4955}{51.46\%} & \colorbox[rgb]{0.3628,0.8406,0.2262}{78.93\%} & \colorbox[rgb]{0.5881,0.8969,0.4998}{51.02\%} & \colorbox[rgb]{0.7666,0.9416,0.7166}{28.91\%} & \colorbox[rgb]{0.7907,0.9476,0.7458}{25.93\%} & \colorbox[rgb]{0.9477,0.9869,0.9365}{6.48\%} & \colorbox[rgb]{0.4951,0.8737,0.3869}{62.54\%} & \colorbox[rgb]{0.6250,0.9062,0.5446}{46.45\%} & \colorbox[rgb]{0.5500,0.8874,0.4535}{55.74\%} & \colorbox[rgb]{0.7268,0.9316,0.6682}{33.84\%} & \colorbox[rgb]{0.6315,0.9078,0.5525}{45.64\%} & \colorbox[rgb]{0.4419,0.8604,0.3222}{69.13\%} & \colorbox[rgb]{0.7461,0.9365,0.6917}{31.45\%} & \colorbox[rgb]{0.7751,0.9437,0.7269}{27.86\%} \\
% 16 & Code Llama                     & CodeLlama-34b-Instruct         & \colorbox[rgb]{0.5927,0.8981,0.5054}{50.45\%} & \colorbox[rgb]{0.4139,0.8533,0.2882}{72.60\%} & \colorbox[rgb]{0.5554,0.8888,0.4601}{55.07\%} & \colorbox[rgb]{0.7323,0.9330,0.6749}{33.16\%} & \colorbox[rgb]{0.8512,0.9628,0.8193}{18.43\%} & \colorbox[rgb]{0.9215,0.9804,0.9047}{9.72\%} & \colorbox[rgb]{0.5825,0.8955,0.4930}{51.71\%} & \colorbox[rgb]{0.6095,0.9023,0.5258}{48.37\%} & \colorbox[rgb]{0.5046,0.8761,0.3984}{61.36\%} & \colorbox[rgb]{0.7010,0.9252,0.6369}{37.04\%} & \colorbox[rgb]{0.6114,0.9028,0.5280}{48.14\%} & \colorbox[rgb]{0.5867,0.8966,0.4980}{51.20\%} & \colorbox[rgb]{0.6144,0.9035,0.5318}{47.76\%} & \colorbox[rgb]{0.7695,0.9423,0.7201}{28.55\%} \\
% 17 & 01.AI                          & Yi-34B-Chat                    & \colorbox[rgb]{0.5997,0.8998,0.5139}{49.58\%} & \colorbox[rgb]{0.3799,0.8448,0.2470}{76.81\%} & \colorbox[rgb]{0.6194,0.9048,0.5377}{47.15\%} & \colorbox[rgb]{0.7633,0.9408,0.7125}{29.32\%} & \colorbox[rgb]{0.7870,0.9467,0.7413}{26.39\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.6440,0.9109,0.5676}{44.10\%} & \colorbox[rgb]{0.6387,0.9096,0.5613}{44.75\%} & \colorbox[rgb]{0.4971,0.8742,0.3893}{62.29\%} & \colorbox[rgb]{0.5976,0.8993,0.5114}{49.84\%} & \colorbox[rgb]{0.5710,0.8927,0.4790}{53.14\%} & \colorbox[rgb]{0.7142,0.9285,0.6529}{35.40\%} & \colorbox[rgb]{0.7082,0.9270,0.6456}{36.15\%} & \colorbox[rgb]{0.7330,0.9332,0.6758}{33.07\%} \\
% 18 & WizardLM                       & WizardCoder-Python-7B-V1.0     & \colorbox[rgb]{0.6036,0.9008,0.5186}{49.10\%} & \colorbox[rgb]{0.3831,0.8456,0.2508}{76.42\%} & \colorbox[rgb]{0.6119,0.9029,0.5286}{48.08\%} & \colorbox[rgb]{0.7652,0.9412,0.7148}{29.09\%} & \colorbox[rgb]{0.8991,0.9748,0.8774}{12.50\%} & \colorbox[rgb]{0.9215,0.9804,0.9047}{9.72\%} & \colorbox[rgb]{0.5269,0.8816,0.4255}{58.60\%} & \colorbox[rgb]{0.6639,0.9159,0.5919}{41.63\%} & \colorbox[rgb]{0.5909,0.8976,0.5032}{50.67\%} & \colorbox[rgb]{0.6651,0.9162,0.5932}{41.49\%} & \colorbox[rgb]{0.6256,0.9063,0.5453}{46.38\%} & \colorbox[rgb]{0.5205,0.8800,0.4176}{59.40\%} & \colorbox[rgb]{0.7958,0.9489,0.7520}{25.30\%} & \colorbox[rgb]{0.8143,0.9535,0.7745}{23.00\%} \\
% 19 & WizardLM                       & WizardCoder-Python-13B-V1.0    & \colorbox[rgb]{0.6045,0.9010,0.5197}{48.99\%} & \colorbox[rgb]{0.3848,0.8461,0.2528}{76.21\%} & \colorbox[rgb]{0.6225,0.9055,0.5416}{46.76\%} & \colorbox[rgb]{0.7240,0.9309,0.6648}{34.19\%} & \colorbox[rgb]{0.8695,0.9673,0.8415}{16.17\%} & \colorbox[rgb]{0.9972,0.9993,0.9966}{0.35\%} & \colorbox[rgb]{0.5746,0.8936,0.4834}{52.69\%} & \colorbox[rgb]{0.6102,0.9025,0.5266}{48.29\%} & \colorbox[rgb]{0.5909,0.8976,0.5032}{50.67\%} & \colorbox[rgb]{0.6664,0.9165,0.5949}{41.32\%} & \colorbox[rgb]{0.6068,0.9016,0.5224}{48.71\%} & \colorbox[rgb]{0.5662,0.8915,0.4732}{53.73\%} & \colorbox[rgb]{0.8349,0.9587,0.7995}{20.45\%} & \colorbox[rgb]{0.7610,0.9402,0.7097}{29.61\%} \\
% 20 & Code Llama                     & CodeLlama-34b                  & \colorbox[rgb]{0.6177,0.9043,0.5357}{47.36\%} & \colorbox[rgb]{0.4182,0.8544,0.2934}{72.07\%} & \colorbox[rgb]{0.6501,0.9125,0.5751}{43.34\%} & \colorbox[rgb]{0.7633,0.9408,0.7125}{29.32\%} & \colorbox[rgb]{0.8289,0.9572,0.7922}{21.20\%} & \colorbox[rgb]{0.8907,0.9726,0.8673}{13.54\%} & \colorbox[rgb]{0.5662,0.8914,0.4731}{53.74\%} & \colorbox[rgb]{0.5956,0.8988,0.5089}{50.09\%} & \colorbox[rgb]{0.5841,0.8959,0.4949}{51.52\%} & \colorbox[rgb]{0.7853,0.9463,0.7393}{26.59\%} & \colorbox[rgb]{0.6514,0.9128,0.5767}{43.18\%} & \colorbox[rgb]{0.5372,0.8842,0.4379}{57.33\%} & \colorbox[rgb]{0.6983,0.9245,0.6336}{37.37\%} & \colorbox[rgb]{0.7994,0.9498,0.7564}{24.85\%} \\
% 21 & Code Llama                     & CodeLlama-13b-Instruct         & \colorbox[rgb]{0.6257,0.9063,0.5454}{46.37\%} & \colorbox[rgb]{0.4424,0.8605,0.3228}{69.07\%} & \colorbox[rgb]{0.6287,0.9071,0.5491}{45.99\%} & \colorbox[rgb]{0.7225,0.9306,0.6630}{34.37\%} & \colorbox[rgb]{0.9078,0.9769,0.8880}{11.42\%} & \colorbox[rgb]{0.9393,0.9848,0.9263}{7.52\%} & \colorbox[rgb]{0.6072,0.9017,0.5230}{48.65\%} & \colorbox[rgb]{0.6353,0.9087,0.5571}{45.18\%} & \colorbox[rgb]{0.5990,0.8997,0.5130}{49.67\%} & \colorbox[rgb]{0.6785,0.9195,0.6095}{39.83\%} & \colorbox[rgb]{0.6148,0.9036,0.5323}{47.71\%} & \colorbox[rgb]{0.5926,0.8981,0.5052}{50.47\%} & \colorbox[rgb]{0.8313,0.9578,0.7951}{20.90\%} & \colorbox[rgb]{0.8995,0.9749,0.8779}{12.45\%} \\
% 22 & Zephyr                         & Zephyr 7B beta                 & \colorbox[rgb]{0.6261,0.9065,0.5460}{46.31\%} & \colorbox[rgb]{0.4477,0.8618,0.3293}{68.41\%} & \colorbox[rgb]{0.5964,0.8990,0.5099}{49.99\%} & \colorbox[rgb]{0.7488,0.9372,0.6950}{31.11\%} & \colorbox[rgb]{0.8790,0.9697,0.8530}{14.99\%} & \colorbox[rgb]{0.9710,0.9927,0.9648}{3.59\%} & \colorbox[rgb]{0.6427,0.9106,0.5661}{44.26\%} & \colorbox[rgb]{0.6378,0.9094,0.5602}{44.86\%} & \colorbox[rgb]{0.5569,0.8891,0.4619}{54.89\%} & \colorbox[rgb]{0.6702,0.9175,0.5995}{40.85\%} & \colorbox[rgb]{0.6022,0.9005,0.5169}{49.28\%} & \colorbox[rgb]{0.7169,0.9292,0.6562}{35.07\%} & \colorbox[rgb]{0.7747,0.9436,0.7264}{27.91\%} & \colorbox[rgb]{0.7767,0.9441,0.7288}{27.66\%} \\
% 23 & DeepSeek MoE                   & deepseek-moe-16b-chat          & \colorbox[rgb]{0.6353,0.9087,0.5571}{45.18\%} & \colorbox[rgb]{0.4498,0.8623,0.3319}{68.15\%} & \colorbox[rgb]{0.6228,0.9056,0.5420}{46.72\%} & \colorbox[rgb]{0.7776,0.9443,0.7299}{27.55\%} & \colorbox[rgb]{0.9179,0.9795,0.9003}{10.17\%} & \colorbox[rgb]{0.9093,0.9773,0.8899}{11.23\%} & \colorbox[rgb]{0.6190,0.9047,0.5373}{47.19\%} & \colorbox[rgb]{0.6243,0.9060,0.5437}{46.54\%} & \colorbox[rgb]{0.6320,0.9079,0.5531}{45.58\%} & \colorbox[rgb]{0.6844,0.9210,0.6168}{39.09\%} & \colorbox[rgb]{0.6310,0.9077,0.5519}{45.71\%} & \colorbox[rgb]{0.6389,0.9096,0.5615}{44.73\%} & \colorbox[rgb]{0.7913,0.9478,0.7466}{25.85\%} & \colorbox[rgb]{0.8329,0.9582,0.7971}{20.70\%} \\
% 24 & OctoPack                       & OctoCoder                      & \colorbox[rgb]{0.6403,0.9100,0.5632}{44.55\%} & \colorbox[rgb]{0.4495,0.8623,0.3315}{68.19\%} & \colorbox[rgb]{0.6641,0.9159,0.5921}{41.61\%} & \colorbox[rgb]{0.7627,0.9406,0.7119}{29.39\%} & \colorbox[rgb]{0.8954,0.9738,0.8729}{12.96\%} & \colorbox[rgb]{0.9103,0.9776,0.8911}{11.11\%} & \colorbox[rgb]{0.6241,0.9059,0.5435}{46.56\%} & \colorbox[rgb]{0.6963,0.9240,0.6312}{37.62\%} & \colorbox[rgb]{0.5675,0.8918,0.4748}{53.57\%} & \colorbox[rgb]{0.6806,0.9201,0.6122}{39.56\%} & \colorbox[rgb]{0.6433,0.9108,0.5669}{44.18\%} & \colorbox[rgb]{0.6200,0.9049,0.5385}{47.07\%} & \colorbox[rgb]{0.8378,0.9594,0.8030}{20.09\%} & \colorbox[rgb]{0.6835,0.9208,0.6157}{39.20\%} \\
% 25 & Qwen                           & Qwen-14B                       & \colorbox[rgb]{0.6473,0.9117,0.5717}{43.69\%} & \colorbox[rgb]{0.4542,0.8634,0.3372}{67.61\%} & \colorbox[rgb]{0.6154,0.9038,0.5329}{47.64\%} & \colorbox[rgb]{0.8234,0.9558,0.7856}{21.87\%} & \colorbox[rgb]{0.9223,0.9805,0.9056}{9.63\%} & \colorbox[rgb]{0.9393,0.9848,0.9263}{7.52\%} & \colorbox[rgb]{0.6400,0.9099,0.5628}{44.59\%} & \colorbox[rgb]{0.6597,0.9149,0.5868}{42.15\%} & \colorbox[rgb]{0.6198,0.9049,0.5383}{47.09\%} & \colorbox[rgb]{0.6772,0.9192,0.6079}{39.99\%} & \colorbox[rgb]{0.6641,0.9159,0.5921}{41.61\%} & \colorbox[rgb]{0.6416,0.9103,0.5647}{44.40\%} & \colorbox[rgb]{0.7240,0.9309,0.6648}{34.19\%} & \colorbox[rgb]{0.7723,0.9430,0.7234}{28.21\%} \\
% 26 & Qwen                           & Qwen-14B-Chat                  & \colorbox[rgb]{0.6489,0.9122,0.5736}{43.49\%} & \colorbox[rgb]{0.4437,0.8608,0.3244}{68.91\%} & \colorbox[rgb]{0.7074,0.9268,0.6446}{36.25\%} & \colorbox[rgb]{0.7761,0.9440,0.7281}{27.73\%} & \colorbox[rgb]{0.9170,0.9792,0.8992}{10.28\%} & \colorbox[rgb]{0.8758,0.9689,0.8491}{15.39\%} & \colorbox[rgb]{0.6336,0.9083,0.5550}{45.39\%} & \colorbox[rgb]{0.6600,0.9149,0.5871}{42.12\%} & \colorbox[rgb]{0.6260,0.9064,0.5458}{46.33\%} & \colorbox[rgb]{0.6894,0.9223,0.6227}{38.48\%} & \colorbox[rgb]{0.6620,0.9154,0.5895}{41.87\%} & \colorbox[rgb]{0.6550,0.9137,0.5811}{42.73\%} & \colorbox[rgb]{0.7079,0.9269,0.6453}{36.18\%} & \colorbox[rgb]{0.7191,0.9297,0.6589}{34.79\%} \\
% 27 & Magicoder                      & Magicoder-DS-6.7B              & \colorbox[rgb]{0.6491,0.9122,0.5738}{43.47\%} & \colorbox[rgb]{0.4588,0.8646,0.3427}{67.04\%} & \colorbox[rgb]{0.6098,0.9024,0.5262}{48.33\%} & \colorbox[rgb]{0.8134,0.9533,0.7734}{23.11\%} & \colorbox[rgb]{0.8899,0.9724,0.8663}{13.64\%} & \colorbox[rgb]{0.9944,0.9986,0.9932}{0.69\%} & \colorbox[rgb]{0.5743,0.8935,0.4830}{52.73\%} & \colorbox[rgb]{0.6737,0.9184,0.6037}{40.42\%} & \colorbox[rgb]{0.6114,0.9028,0.5280}{48.14\%} & \colorbox[rgb]{0.7933,0.9483,0.7489}{25.61\%} & \colorbox[rgb]{0.6902,0.9225,0.6238}{38.37\%} & \colorbox[rgb]{0.5420,0.8854,0.4438}{56.73\%} & \colorbox[rgb]{0.7593,0.9398,0.7077}{29.81\%} & \colorbox[rgb]{0.6927,0.9231,0.6268}{38.07\%} \\
% 28 & Code Llama                     & CodeLlama-34b-Python           & \colorbox[rgb]{0.6518,0.9129,0.5772}{43.13\%} & \colorbox[rgb]{0.4670,0.8666,0.3527}{66.02\%} & \colorbox[rgb]{0.6709,0.9177,0.6004}{40.76\%} & \colorbox[rgb]{0.7089,0.9272,0.6465}{36.06\%} & \colorbox[rgb]{0.9440,0.9860,0.9320}{6.94\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.5952,0.8987,0.5084}{50.14\%} & \colorbox[rgb]{0.6732,0.9182,0.6031}{40.48\%} & \colorbox[rgb]{0.6477,0.9118,0.5722}{43.64\%} & \colorbox[rgb]{0.7245,0.9311,0.6654}{34.13\%} & \colorbox[rgb]{0.6739,0.9184,0.6039}{40.40\%} & \colorbox[rgb]{0.5883,0.8970,0.5000}{51.00\%} & \colorbox[rgb]{0.7769,0.9442,0.7291}{27.63\%} & \colorbox[rgb]{0.8654,0.9663,0.8366}{16.67\%} \\
% 29 & Code Llama                     & CodeLlama-70b-Instruct         & \colorbox[rgb]{0.6543,0.9135,0.5802}{42.82\%} & \colorbox[rgb]{0.5230,0.8807,0.4208}{59.08\%} & \colorbox[rgb]{0.6437,0.9108,0.5673}{44.14\%} & \colorbox[rgb]{0.6894,0.9223,0.6227}{38.48\%} & \colorbox[rgb]{0.9013,0.9753,0.8802}{12.22\%} & \colorbox[rgb]{0.9383,0.9846,0.9251}{7.64\%} & \colorbox[rgb]{0.6916,0.9228,0.6255}{38.20\%} & \colorbox[rgb]{0.6368,0.9091,0.5589}{44.99\%} & \colorbox[rgb]{0.6216,0.9053,0.5405}{46.87\%} & \colorbox[rgb]{0.6579,0.9144,0.5845}{42.38\%} & \colorbox[rgb]{0.6098,0.9024,0.5261}{48.34\%} & \colorbox[rgb]{0.7417,0.9354,0.6863}{32.00\%} & \colorbox[rgb]{0.8701,0.9675,0.8423}{16.09\%} & \colorbox[rgb]{0.9546,0.9886,0.9449}{5.62\%} \\
% 30 & Magicoder                      & Magicoder-CL-7B                & \colorbox[rgb]{0.6633,0.9157,0.5911}{41.71\%} & \colorbox[rgb]{0.4318,0.8578,0.3100}{70.38\%} & \colorbox[rgb]{0.7055,0.9263,0.6424}{36.48\%} & \colorbox[rgb]{0.8138,0.9534,0.7739}{23.06\%} & \colorbox[rgb]{0.9166,0.9791,0.8987}{10.33\%} & \colorbox[rgb]{0.9972,0.9993,0.9966}{0.35\%} & \colorbox[rgb]{0.6023,0.9005,0.5171}{49.26\%} & \colorbox[rgb]{0.7166,0.9291,0.6558}{35.11\%} & \colorbox[rgb]{0.6334,0.9083,0.5548}{45.41\%} & \colorbox[rgb]{0.7298,0.9324,0.6719}{33.47\%} & \colorbox[rgb]{0.6944,0.9235,0.6289}{37.85\%} & \colorbox[rgb]{0.5780,0.8944,0.4875}{52.27\%} & \colorbox[rgb]{0.8393,0.9598,0.8048}{19.91\%} & \colorbox[rgb]{0.6835,0.9208,0.6156}{39.21\%} \\
% 31 & Code Llama                     & CodeLlama-13b                  & \colorbox[rgb]{0.6637,0.9158,0.5916}{41.66\%} & \colorbox[rgb]{0.4933,0.8732,0.3846}{62.77\%} & \colorbox[rgb]{0.6739,0.9184,0.6039}{40.40\%} & \colorbox[rgb]{0.7488,0.9372,0.6950}{31.11\%} & \colorbox[rgb]{0.9357,0.9839,0.9219}{7.97\%} & \colorbox[rgb]{0.9402,0.9850,0.9274}{7.41\%} & \colorbox[rgb]{0.6919,0.9229,0.6258}{38.17\%} & \colorbox[rgb]{0.6403,0.9100,0.5631}{44.56\%} & \colorbox[rgb]{0.6529,0.9131,0.5784}{43.00\%} & \colorbox[rgb]{0.6632,0.9157,0.5910}{41.72\%} & \colorbox[rgb]{0.6332,0.9082,0.5545}{45.44\%} & \colorbox[rgb]{0.7191,0.9297,0.6588}{34.80\%} & \colorbox[rgb]{0.8806,0.9701,0.8550}{14.79\%} & \colorbox[rgb]{0.9801,0.9950,0.9758}{2.47\%} \\
% 32 & DeepSeek Coder                 & deepseek-coder-1.3b-instruct   & \colorbox[rgb]{0.6664,0.9165,0.5949}{41.32\%} & \colorbox[rgb]{0.4714,0.8677,0.3580}{65.48\%} & \colorbox[rgb]{0.6656,0.9163,0.5939}{41.42\%} & \colorbox[rgb]{0.7943,0.9485,0.7502}{25.48\%} & \colorbox[rgb]{0.9491,0.9873,0.9382}{6.30\%} & \colorbox[rgb]{0.9776,0.9944,0.9727}{2.78\%} & \colorbox[rgb]{0.6617,0.9153,0.5891}{41.91\%} & \colorbox[rgb]{0.6564,0.9140,0.5827}{42.56\%} & \colorbox[rgb]{0.6538,0.9134,0.5796}{42.88\%} & \colorbox[rgb]{0.7063,0.9265,0.6433}{36.38\%} & \colorbox[rgb]{0.6625,0.9156,0.5902}{41.80\%} & \colorbox[rgb]{0.6593,0.9148,0.5863}{42.20\%} & \colorbox[rgb]{0.8666,0.9666,0.8380}{16.52\%} & \colorbox[rgb]{0.8037,0.9509,0.7616}{24.32\%} \\
% 33 & Code Llama                     & CodeLlama-13b-Python           & \colorbox[rgb]{0.6665,0.9166,0.5950}{41.31\%} & \colorbox[rgb]{0.4920,0.8729,0.3830}{62.93\%} & \colorbox[rgb]{0.6706,0.9176,0.6000}{40.80\%} & \colorbox[rgb]{0.7690,0.9422,0.7195}{28.61\%} & \colorbox[rgb]{0.9163,0.9791,0.8983}{10.37\%} & \colorbox[rgb]{0.9579,0.9895,0.9489}{5.21\%} & \colorbox[rgb]{0.5968,0.8991,0.5103}{49.95\%} & \colorbox[rgb]{0.6399,0.9099,0.5627}{44.60\%} & \colorbox[rgb]{0.7039,0.9259,0.6404}{36.68\%} & \colorbox[rgb]{0.7803,0.9450,0.7331}{27.22\%} & \colorbox[rgb]{0.6724,0.9180,0.6022}{40.58\%} & \colorbox[rgb]{0.5877,0.8968,0.4993}{51.07\%} & \colorbox[rgb]{0.9038,0.9759,0.8831}{11.92\%} & \colorbox[rgb]{0.8899,0.9724,0.8663}{13.64\%} \\
% 34 & WizardLM                       & WizardCoder-15B-V1.0           & \colorbox[rgb]{0.6689,0.9172,0.5979}{41.01\%} & \colorbox[rgb]{0.4656,0.8663,0.3511}{66.19\%} & \colorbox[rgb]{0.6743,0.9185,0.6045}{40.34\%} & \colorbox[rgb]{0.8247,0.9561,0.7871}{21.72\%} & \colorbox[rgb]{0.8997,0.9749,0.8782}{12.42\%} & \colorbox[rgb]{0.9860,0.9965,0.9829}{1.74\%} & \colorbox[rgb]{0.6383,0.9095,0.5608}{44.80\%} & \colorbox[rgb]{0.7212,0.9302,0.6614}{34.54\%} & \colorbox[rgb]{0.6151,0.9037,0.5325}{47.68\%} & \colorbox[rgb]{0.7151,0.9287,0.6540}{35.29\%} & \colorbox[rgb]{0.6898,0.9224,0.6232}{38.43\%} & \colorbox[rgb]{0.6157,0.9038,0.5333}{47.60\%} & \colorbox[rgb]{0.8199,0.9549,0.7813}{22.31\%} & \colorbox[rgb]{0.7174,0.9293,0.6568}{35.01\%} \\
% 35 & Code Llama                     & CodeLlama-70b                  & \colorbox[rgb]{0.6722,0.9180,0.6020}{40.60\%} & \colorbox[rgb]{0.5109,0.8776,0.4060}{60.59\%} & \colorbox[rgb]{0.6979,0.9244,0.6331}{37.42\%} & \colorbox[rgb]{0.7120,0.9279,0.6502}{35.68\%} & \colorbox[rgb]{0.9387,0.9847,0.9256}{7.59\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.6191,0.9047,0.5374}{47.18\%} & \colorbox[rgb]{0.6843,0.9210,0.6167}{39.10\%} & \colorbox[rgb]{0.6844,0.9210,0.6168}{39.09\%} & \colorbox[rgb]{0.7319,0.9329,0.6744}{33.21\%} & \colorbox[rgb]{0.6727,0.9181,0.6025}{40.54\%} & \colorbox[rgb]{0.6367,0.9091,0.5588}{45.00\%} & \colorbox[rgb]{0.8448,0.9612,0.8115}{19.23\%} & \colorbox[rgb]{0.9309,0.9827,0.9161}{8.56\%} \\
% 36 & Code Llama                     & CodeLlama-70b-Python           & \colorbox[rgb]{0.6747,0.9186,0.6050}{40.29\%} & \colorbox[rgb]{0.5226,0.8805,0.4202}{59.14\%} & \colorbox[rgb]{0.7088,0.9271,0.6464}{36.07\%} & \colorbox[rgb]{0.6685,0.9171,0.5974}{41.06\%} & \colorbox[rgb]{0.9387,0.9847,0.9256}{7.59\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.6607,0.9151,0.5879}{42.03\%} & \colorbox[rgb]{0.6525,0.9131,0.5780}{43.04\%} & \colorbox[rgb]{0.6709,0.9177,0.6004}{40.76\%} & \colorbox[rgb]{0.7380,0.9344,0.6818}{32.46\%} & \colorbox[rgb]{0.6627,0.9156,0.5904}{41.78\%} & \colorbox[rgb]{0.6690,0.9172,0.5980}{41.00\%} & \colorbox[rgb]{0.9115,0.9779,0.8925}{10.96\%} & \colorbox[rgb]{0.8426,0.9606,0.8088}{19.50\%} \\
% 37 & OctoPack                       & OctoGeeX                       & \colorbox[rgb]{0.6759,0.9189,0.6065}{40.14\%} & \colorbox[rgb]{0.4951,0.8737,0.3869}{62.54\%} & \colorbox[rgb]{0.6945,0.9236,0.6290}{37.84\%} & \colorbox[rgb]{0.7870,0.9467,0.7413}{26.39\%} & \colorbox[rgb]{0.8735,0.9683,0.8464}{15.67\%} & \colorbox[rgb]{0.9822,0.9956,0.9784}{2.20\%} & \colorbox[rgb]{0.6590,0.9147,0.5859}{42.24\%} & \colorbox[rgb]{0.7317,0.9329,0.6742}{33.23\%} & \colorbox[rgb]{0.6285,0.9070,0.5488}{46.02\%} & \colorbox[rgb]{0.6843,0.9210,0.6167}{39.10\%} & \colorbox[rgb]{0.6783,0.9195,0.6093}{39.85\%} & \colorbox[rgb]{0.6774,0.9193,0.6082}{39.96\%} & \colorbox[rgb]{0.8313,0.9578,0.7951}{20.90\%} & \colorbox[rgb]{0.7488,0.9372,0.6950}{31.11\%} \\
% 38 & DeepSeek LLM                   & deepseek-llm-67b-base          & \colorbox[rgb]{0.6781,0.9195,0.6091}{39.87\%} & \colorbox[rgb]{0.5386,0.8846,0.4397}{57.15\%} & \colorbox[rgb]{0.6066,0.9016,0.5223}{48.73\%} & \colorbox[rgb]{0.8037,0.9509,0.7616}{24.32\%} & \colorbox[rgb]{0.9260,0.9815,0.9101}{9.17\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.7134,0.9283,0.6520}{35.50\%} & \colorbox[rgb]{0.6515,0.9128,0.5768}{43.17\%} & \colorbox[rgb]{0.6274,0.9068,0.5475}{46.15\%} & \colorbox[rgb]{0.7223,0.9305,0.6627}{34.40\%} & \colorbox[rgb]{0.6772,0.9192,0.6080}{39.98\%} & \colorbox[rgb]{0.7094,0.9273,0.6471}{36.00\%} & \colorbox[rgb]{0.7578,0.9394,0.7059}{30.00\%} & \colorbox[rgb]{0.8025,0.9506,0.7602}{24.46\%} \\
% 39 & Llama 2                        & Llama2-70B-Chat                & \colorbox[rgb]{0.6827,0.9206,0.6147}{39.30\%} & \colorbox[rgb]{0.5402,0.8850,0.4417}{56.95\%} & \colorbox[rgb]{0.6931,0.9232,0.6273}{38.02\%} & \colorbox[rgb]{0.7279,0.9319,0.6695}{33.71\%} & \colorbox[rgb]{0.9357,0.9839,0.9220}{7.96\%} & \colorbox[rgb]{0.9383,0.9846,0.9251}{7.64\%} & \colorbox[rgb]{0.7122,0.9280,0.6505}{35.65\%} & \colorbox[rgb]{0.6539,0.9134,0.5797}{42.87\%} & \colorbox[rgb]{0.6564,0.9140,0.5827}{42.56\%} & \colorbox[rgb]{0.7085,0.9271,0.6460}{36.11\%} & \colorbox[rgb]{0.6699,0.9174,0.5991}{40.89\%} & \colorbox[rgb]{0.7223,0.9305,0.6627}{34.40\%} & \colorbox[rgb]{0.8188,0.9547,0.7800}{22.44\%} & \colorbox[rgb]{0.7728,0.9432,0.7241}{28.14\%} \\
% 40 & DeepSeek Coder                 & deepseek-coder-33b-base        & \colorbox[rgb]{0.6872,0.9217,0.6201}{38.75\%} & \colorbox[rgb]{0.5420,0.8854,0.4438}{56.73\%} & \colorbox[rgb]{0.6403,0.9100,0.5632}{44.55\%} & \colorbox[rgb]{0.8398,0.9599,0.8054}{19.85\%} & \colorbox[rgb]{0.8793,0.9698,0.8534}{14.95\%} & \colorbox[rgb]{0.9328,0.9832,0.9183}{8.33\%} & \colorbox[rgb]{0.7307,0.9326,0.6729}{33.36\%} & \colorbox[rgb]{0.6470,0.9117,0.5713}{43.73\%} & \colorbox[rgb]{0.6282,0.9070,0.5484}{46.06\%} & \colorbox[rgb]{0.7479,0.9369,0.6938}{31.23\%} & \colorbox[rgb]{0.6449,0.9111,0.5687}{43.99\%} & \colorbox[rgb]{0.7941,0.9485,0.7500}{25.50\%} & \colorbox[rgb]{0.8830,0.9707,0.8579}{14.49\%} & \colorbox[rgb]{0.7738,0.9434,0.7253}{28.02\%} \\
% 41 & 01.AI                          & Yi-6B-Chat                     & \colorbox[rgb]{0.6921,0.9230,0.6261}{38.14\%} & \colorbox[rgb]{0.5743,0.8935,0.4830}{52.73\%} & \colorbox[rgb]{0.6916,0.9228,0.6255}{38.20\%} & \colorbox[rgb]{0.7225,0.9306,0.6630}{34.37\%} & \colorbox[rgb]{0.8988,0.9747,0.8772}{12.53\%} & \colorbox[rgb]{0.9383,0.9846,0.9251}{7.64\%} & \colorbox[rgb]{0.7307,0.9326,0.6729}{33.36\%} & \colorbox[rgb]{0.6786,0.9196,0.6097}{39.81\%} & \colorbox[rgb]{0.6566,0.9141,0.5829}{42.54\%} & \colorbox[rgb]{0.6906,0.9226,0.6242}{38.33\%} & \colorbox[rgb]{0.6508,0.9126,0.5759}{43.26\%} & \colorbox[rgb]{0.8076,0.9519,0.7664}{23.83\%} & \colorbox[rgb]{0.8763,0.9691,0.8498}{15.32\%} & \colorbox[rgb]{0.8733,0.9683,0.8462}{15.69\%} \\
% 42 & Llama 2                        & Llama2-70B                     & \colorbox[rgb]{0.6957,0.9239,0.6305}{37.69\%} & \colorbox[rgb]{0.5842,0.8959,0.4950}{51.51\%} & \colorbox[rgb]{0.6563,0.9140,0.5825}{42.58\%} & \colorbox[rgb]{0.7701,0.9425,0.7208}{28.48\%} & \colorbox[rgb]{0.9177,0.9794,0.9001}{10.19\%} & \colorbox[rgb]{0.9159,0.9790,0.8978}{10.42\%} & \colorbox[rgb]{0.7073,0.9268,0.6445}{36.26\%} & \colorbox[rgb]{0.6529,0.9132,0.5785}{42.99\%} & \colorbox[rgb]{0.7003,0.9250,0.6361}{37.12\%} & \colorbox[rgb]{0.7338,0.9334,0.6767}{32.98\%} & \colorbox[rgb]{0.6810,0.9202,0.6125}{39.52\%} & \colorbox[rgb]{0.7740,0.9434,0.7255}{28.00\%} & \colorbox[rgb]{0.7542,0.9385,0.7015}{30.45\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 43 & Code Llama                     & CodeLlama-7b                   & \colorbox[rgb]{0.6963,0.9240,0.6312}{37.62\%} & \colorbox[rgb]{0.5172,0.8792,0.4136}{59.81\%} & \colorbox[rgb]{0.6912,0.9227,0.6250}{38.25\%} & \colorbox[rgb]{0.8436,0.9609,0.8101}{19.37\%} & \colorbox[rgb]{0.9248,0.9812,0.9086}{9.32\%} & \colorbox[rgb]{0.9608,0.9902,0.9524}{4.86\%} & \colorbox[rgb]{0.6594,0.9148,0.5864}{42.19\%} & \colorbox[rgb]{0.6884,0.9220,0.6216}{38.60\%} & \colorbox[rgb]{0.6983,0.9245,0.6336}{37.37\%} & \colorbox[rgb]{0.7706,0.9426,0.7215}{28.41\%} & \colorbox[rgb]{0.6943,0.9235,0.6287}{37.87\%} & \colorbox[rgb]{0.6625,0.9156,0.5902}{41.80\%} & \colorbox[rgb]{0.8779,0.9694,0.8517}{15.13\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 44 & Mistral                        & Mistral-7B-Instruct-v0.1       & \colorbox[rgb]{0.6969,0.9241,0.6319}{37.55\%} & \colorbox[rgb]{0.5454,0.8863,0.4479}{56.31\%} & \colorbox[rgb]{0.6663,0.9165,0.5947}{41.34\%} & \colorbox[rgb]{0.8057,0.9514,0.7640}{24.07\%} & \colorbox[rgb]{0.9397,0.9849,0.9268}{7.47\%} & \colorbox[rgb]{0.9720,0.9930,0.9660}{3.47\%} & \colorbox[rgb]{0.6792,0.9197,0.6104}{39.74\%} & \colorbox[rgb]{0.7518,0.9379,0.6986}{30.74\%} & \colorbox[rgb]{0.6198,0.9049,0.5382}{47.10\%} & \colorbox[rgb]{0.7465,0.9366,0.6922}{31.40\%} & \colorbox[rgb]{0.7241,0.9310,0.6650}{34.17\%} & \colorbox[rgb]{0.6787,0.9196,0.6098}{39.80\%} & \colorbox[rgb]{0.7220,0.9304,0.6624}{34.44\%} & \colorbox[rgb]{0.7586,0.9396,0.7069}{29.90\%} \\
% 45 & InternLM                       & InternLM-Chat-20B              & \colorbox[rgb]{0.6980,0.9244,0.6332}{37.41\%} & \colorbox[rgb]{0.5158,0.8788,0.4120}{59.98\%} & \colorbox[rgb]{0.7392,0.9348,0.6833}{32.30\%} & \colorbox[rgb]{0.8353,0.9588,0.8000}{20.40\%} & \colorbox[rgb]{0.8511,0.9628,0.8192}{18.44\%} & \colorbox[rgb]{0.9430,0.9857,0.9308}{7.06\%} & \colorbox[rgb]{0.6336,0.9083,0.5551}{45.38\%} & \colorbox[rgb]{0.7201,0.9300,0.6601}{34.67\%} & \colorbox[rgb]{0.7235,0.9308,0.6642}{34.25\%} & \colorbox[rgb]{0.7447,0.9361,0.6899}{31.63\%} & \colorbox[rgb]{0.7214,0.9303,0.6617}{34.51\%} & \colorbox[rgb]{0.6270,0.9067,0.5471}{46.20\%} & \colorbox[rgb]{0.8532,0.9633,0.8218}{18.18\%} & \colorbox[rgb]{0.8102,0.9525,0.7695}{23.51\%} \\
% 46 & Qwen                           & Qwen-7B-Chat                   & \colorbox[rgb]{0.6984,0.9245,0.6337}{37.36\%} & \colorbox[rgb]{0.5138,0.8783,0.4095}{60.23\%} & \colorbox[rgb]{0.7078,0.9269,0.6451}{36.20\%} & \colorbox[rgb]{0.8404,0.9601,0.8062}{19.77\%} & \colorbox[rgb]{0.9382,0.9845,0.9250}{7.65\%} & \colorbox[rgb]{0.9524,0.9881,0.9422}{5.90\%} & \colorbox[rgb]{0.6493,0.9123,0.5741}{43.44\%} & \colorbox[rgb]{0.7386,0.9346,0.6825}{32.38\%} & \colorbox[rgb]{0.6914,0.9228,0.6253}{38.22\%} & \colorbox[rgb]{0.7338,0.9334,0.6767}{32.98\%} & \colorbox[rgb]{0.7250,0.9312,0.6661}{34.06\%} & \colorbox[rgb]{0.6523,0.9130,0.5777}{43.07\%} & \colorbox[rgb]{0.7657,0.9414,0.7155}{29.02\%} & \colorbox[rgb]{0.7569,0.9392,0.7048}{30.11\%} \\
% 47 & DeepSeek LLM                   & deepseek-llm-7b-chat           & \colorbox[rgb]{0.7033,0.9258,0.6397}{36.75\%} & \colorbox[rgb]{0.5523,0.8880,0.4563}{55.46\%} & \colorbox[rgb]{0.6821,0.9205,0.6139}{39.38\%} & \colorbox[rgb]{0.8148,0.9537,0.7751}{22.94\%} & \colorbox[rgb]{0.9491,0.9873,0.9382}{6.30\%} & \colorbox[rgb]{0.9486,0.9871,0.9375}{6.37\%} & \colorbox[rgb]{0.7249,0.9312,0.6659}{34.08\%} & \colorbox[rgb]{0.7598,0.9399,0.7083}{29.75\%} & \colorbox[rgb]{0.6225,0.9055,0.5416}{46.76\%} & \colorbox[rgb]{0.6865,0.9216,0.6193}{38.83\%} & \colorbox[rgb]{0.6839,0.9209,0.6162}{39.15\%} & \colorbox[rgb]{0.7568,0.9391,0.7046}{30.13\%} & \colorbox[rgb]{0.8716,0.9679,0.8441}{15.90\%} & \colorbox[rgb]{0.7095,0.9273,0.6473}{35.98\%} \\
% 48 & Llama 2                        & Llama2-7B-Chat                 & \colorbox[rgb]{0.7082,0.9270,0.6457}{36.14\%} & \colorbox[rgb]{0.5627,0.8906,0.4689}{54.17\%} & \colorbox[rgb]{0.7146,0.9286,0.6534}{35.35\%} & \colorbox[rgb]{0.8004,0.9501,0.7576}{24.72\%} & \colorbox[rgb]{0.9238,0.9809,0.9075}{9.44\%} & \colorbox[rgb]{0.9271,0.9818,0.9115}{9.03\%} & \colorbox[rgb]{0.7132,0.9282,0.6517}{35.53\%} & \colorbox[rgb]{0.7312,0.9328,0.6736}{33.29\%} & \colorbox[rgb]{0.6839,0.9209,0.6161}{39.16\%} & \colorbox[rgb]{0.6972,0.9242,0.6323}{37.51\%} & \colorbox[rgb]{0.6961,0.9240,0.6310}{37.64\%} & \colorbox[rgb]{0.7699,0.9424,0.7206}{28.50\%} & \colorbox[rgb]{0.8276,0.9569,0.7907}{21.35\%} & \colorbox[rgb]{0.7759,0.9439,0.7278}{27.76\%} \\
% 49 & WizardLM                       & WizardCoder-3B-V1.0            & \colorbox[rgb]{0.7125,0.9281,0.6509}{35.61\%} & \colorbox[rgb]{0.5363,0.8840,0.4369}{57.44\%} & \colorbox[rgb]{0.7125,0.9281,0.6509}{35.61\%} & \colorbox[rgb]{0.8770,0.9692,0.8507}{15.23\%} & \colorbox[rgb]{0.9088,0.9772,0.8892}{11.30\%} & \colorbox[rgb]{0.9467,0.9867,0.9353}{6.60\%} & \colorbox[rgb]{0.6831,0.9207,0.6152}{39.25\%} & \colorbox[rgb]{0.7410,0.9352,0.6855}{32.08\%} & \colorbox[rgb]{0.6663,0.9165,0.5947}{41.34\%} & \colorbox[rgb]{0.7824,0.9455,0.7357}{26.96\%} & \colorbox[rgb]{0.7107,0.9276,0.6487}{35.83\%} & \colorbox[rgb]{0.7142,0.9285,0.6529}{35.40\%} & \colorbox[rgb]{0.8446,0.9611,0.8113}{19.25\%} & \colorbox[rgb]{0.7861,0.9465,0.7402}{26.50\%} \\
% 50 & Code Llama                     & CodeLlama-7b-Instruct          & \colorbox[rgb]{0.7162,0.9290,0.6554}{35.15\%} & \colorbox[rgb]{0.5666,0.8915,0.4736}{53.69\%} & \colorbox[rgb]{0.7111,0.9277,0.6491}{35.79\%} & \colorbox[rgb]{0.7996,0.9499,0.7567}{24.82\%} & \colorbox[rgb]{0.9387,0.9847,0.9256}{7.59\%} & \colorbox[rgb]{0.9888,0.9972,0.9864}{1.39\%} & \colorbox[rgb]{0.7057,0.9264,0.6425}{36.46\%} & \colorbox[rgb]{0.7002,0.9250,0.6360}{37.13\%} & \colorbox[rgb]{0.7174,0.9293,0.6569}{35.00\%} & \colorbox[rgb]{0.7574,0.9393,0.7054}{30.05\%} & \colorbox[rgb]{0.7096,0.9273,0.6474}{35.97\%} & \colorbox[rgb]{0.7185,0.9296,0.6581}{34.87\%} & \colorbox[rgb]{0.8727,0.9681,0.8454}{15.77\%} & \colorbox[rgb]{0.8884,0.9721,0.8644}{13.83\%} \\
% 51 & InternLM                       & InternLM-Chat-7B               & \colorbox[rgb]{0.7186,0.9296,0.6582}{34.86\%} & \colorbox[rgb]{0.5495,0.8873,0.4529}{55.80\%} & \colorbox[rgb]{0.7385,0.9346,0.6824}{32.39\%} & \colorbox[rgb]{0.8324,0.9581,0.7965}{20.76\%} & \colorbox[rgb]{0.8975,0.9743,0.8755}{12.70\%} & \colorbox[rgb]{0.9851,0.9963,0.9819}{1.85\%} & \colorbox[rgb]{0.7149,0.9287,0.6538}{35.31\%} & \colorbox[rgb]{0.7231,0.9307,0.6637}{34.30\%} & \colorbox[rgb]{0.6791,0.9197,0.6103}{39.75\%} & \colorbox[rgb]{0.7698,0.9424,0.7204}{28.52\%} & \colorbox[rgb]{0.7156,0.9288,0.6546}{35.23\%} & \colorbox[rgb]{0.7209,0.9302,0.6611}{34.57\%} & \colorbox[rgb]{0.8575,0.9643,0.8270}{17.65\%} & \colorbox[rgb]{0.8639,0.9659,0.8347}{16.86\%} \\
% 52 & Baichuan2                      & Baichuan2-13B-Chat             & \colorbox[rgb]{0.7223,0.9305,0.6627}{34.40\%} & \colorbox[rgb]{0.5659,0.8914,0.4728}{53.77\%} & \colorbox[rgb]{0.7765,0.9441,0.7285}{27.69\%} & \colorbox[rgb]{0.8047,0.9511,0.7628}{24.19\%} & \colorbox[rgb]{0.9447,0.9862,0.9328}{6.85\%} & \colorbox[rgb]{0.8860,0.9715,0.8616}{14.12\%} & \colorbox[rgb]{0.7011,0.9252,0.6370}{37.03\%} & \colorbox[rgb]{0.7099,0.9274,0.6477}{35.93\%} & \colorbox[rgb]{0.7062,0.9265,0.6432}{36.39\%} & \colorbox[rgb]{0.7991,0.9497,0.7561}{24.88\%} & \colorbox[rgb]{0.7205,0.9301,0.6606}{34.62\%} & \colorbox[rgb]{0.7492,0.9372,0.6954}{31.07\%} & \colorbox[rgb]{0.8173,0.9543,0.7781}{22.63\%} & \colorbox[rgb]{0.8524,0.9631,0.8208}{18.28\%} \\
% 53 & DeepSeek Coder                 & deepseek-coder-6.7b-base       & \colorbox[rgb]{0.7283,0.9320,0.6700}{33.66\%} & \colorbox[rgb]{0.5700,0.8924,0.4778}{53.26\%} & \colorbox[rgb]{0.6936,0.9233,0.6279}{37.95\%} & \colorbox[rgb]{0.8868,0.9717,0.8625}{14.02\%} & \colorbox[rgb]{0.9309,0.9827,0.9161}{8.56\%} & \colorbox[rgb]{0.9776,0.9944,0.9727}{2.78\%} & \colorbox[rgb]{0.7049,0.9261,0.6416}{36.56\%} & \colorbox[rgb]{0.7384,0.9346,0.6824}{32.40\%} & \colorbox[rgb]{0.6946,0.9236,0.6291}{37.83\%} & \colorbox[rgb]{0.7982,0.9495,0.7549}{25.00\%} & \colorbox[rgb]{0.7161,0.9290,0.6552}{35.17\%} & \colorbox[rgb]{0.7298,0.9324,0.6719}{33.47\%} & \colorbox[rgb]{0.9038,0.9759,0.8831}{11.92\%} & \colorbox[rgb]{0.9289,0.9822,0.9136}{8.81\%} \\
% 54 & Code Llama                     & CodeLlama-7b-Python            & \colorbox[rgb]{0.7345,0.9336,0.6775}{32.89\%} & \colorbox[rgb]{0.5881,0.8969,0.4998}{51.02\%} & \colorbox[rgb]{0.7684,0.9420,0.7187}{28.69\%} & \colorbox[rgb]{0.8037,0.9509,0.7616}{24.32\%} & \colorbox[rgb]{0.9387,0.9847,0.9256}{7.59\%} & \colorbox[rgb]{0.9440,0.9860,0.9320}{6.94\%} & \colorbox[rgb]{0.7547,0.9386,0.7022}{30.38\%} & \colorbox[rgb]{0.6905,0.9226,0.6241}{38.34\%} & \colorbox[rgb]{0.7387,0.9346,0.6826}{32.37\%} & \colorbox[rgb]{0.7593,0.9398,0.7077}{29.81\%} & \colorbox[rgb]{0.7153,0.9288,0.6542}{35.27\%} & \colorbox[rgb]{0.7546,0.9386,0.7020}{30.40\%} & \colorbox[rgb]{0.9276,0.9819,0.9121}{8.97\%} & \colorbox[rgb]{0.9087,0.9772,0.8891}{11.31\%} \\
% 55 & Llama 2                        & Llama2-13B-Chat                & \colorbox[rgb]{0.7393,0.9348,0.6834}{32.29\%} & \colorbox[rgb]{0.5867,0.8966,0.4981}{51.19\%} & \colorbox[rgb]{0.7644,0.9411,0.7139}{29.18\%} & \colorbox[rgb]{0.8159,0.9539,0.7765}{22.80\%} & \colorbox[rgb]{0.9387,0.9847,0.9256}{7.59\%} & \colorbox[rgb]{0.9832,0.9958,0.9796}{2.08\%} & \colorbox[rgb]{0.7779,0.9444,0.7303}{27.51\%} & \colorbox[rgb]{0.7660,0.9415,0.7159}{28.98\%} & \colorbox[rgb]{0.6540,0.9134,0.5798}{42.86\%} & \colorbox[rgb]{0.7430,0.9357,0.6878}{31.84\%} & \colorbox[rgb]{0.7007,0.9251,0.6366}{37.07\%} & \colorbox[rgb]{0.8299,0.9574,0.7934}{21.07\%} & \colorbox[rgb]{0.9260,0.9815,0.9101}{9.17\%} & \colorbox[rgb]{0.8404,0.9601,0.8062}{19.77\%} \\
% 56 & WizardLM                       & WizardCoder-1B-V1.0            & \colorbox[rgb]{0.7421,0.9355,0.6869}{31.94\%} & \colorbox[rgb]{0.6214,0.9053,0.5402}{46.90\%} & \colorbox[rgb]{0.7578,0.9394,0.7059}{30.00\%} & \colorbox[rgb]{0.7790,0.9447,0.7317}{27.37\%} & \colorbox[rgb]{0.9890,0.9973,0.9867}{1.36\%} & \colorbox[rgb]{0.9215,0.9804,0.9047}{9.72\%} & \colorbox[rgb]{0.7679,0.9419,0.7181}{28.75\%} & \colorbox[rgb]{0.7516,0.9378,0.6983}{30.77\%} & \colorbox[rgb]{0.7029,0.9257,0.6392}{36.80\%} & \colorbox[rgb]{0.7341,0.9335,0.6771}{32.94\%} & \colorbox[rgb]{0.7215,0.9303,0.6618}{34.50\%} & \colorbox[rgb]{0.7982,0.9495,0.7549}{25.00\%} & \colorbox[rgb]{0.8656,0.9664,0.8368}{16.65\%} & \colorbox[rgb]{0.8330,0.9582,0.7972}{20.69\%} \\
% 57 & Qwen                           & Qwen-7B                        & \colorbox[rgb]{0.7442,0.9360,0.6893}{31.69\%} & \colorbox[rgb]{0.5750,0.8936,0.4838}{52.65\%} & \colorbox[rgb]{0.7402,0.9350,0.6845}{32.18\%} & \colorbox[rgb]{0.8775,0.9693,0.8512}{15.18\%} & \colorbox[rgb]{0.9830,0.9958,0.9794}{2.10\%} & \colorbox[rgb]{0.9851,0.9963,0.9819}{1.85\%} & \colorbox[rgb]{0.7273,0.9318,0.6688}{33.78\%} & \colorbox[rgb]{0.7521,0.9380,0.6989}{30.71\%} & \colorbox[rgb]{0.7031,0.9257,0.6394}{36.78\%} & \colorbox[rgb]{0.8157,0.9539,0.7762}{22.83\%} & \colorbox[rgb]{0.7490,0.9372,0.6952}{31.09\%} & \colorbox[rgb]{0.7250,0.9312,0.6660}{34.07\%} & \colorbox[rgb]{0.8732,0.9683,0.8460}{15.71\%} & \colorbox[rgb]{0.8618,0.9654,0.8322}{17.12\%} \\
% 58 & StarCoder                      & StarCode+                      & \colorbox[rgb]{0.7524,0.9380,0.6993}{30.67\%} & \colorbox[rgb]{0.5884,0.8970,0.5001}{50.99\%} & \colorbox[rgb]{0.7618,0.9404,0.7107}{29.51\%} & \colorbox[rgb]{0.8846,0.9711,0.8599}{14.29\%} & \colorbox[rgb]{0.9676,0.9919,0.9607}{4.01\%} & \colorbox[rgb]{0.9626,0.9906,0.9546}{4.63\%} & \colorbox[rgb]{0.7430,0.9357,0.6879}{31.83\%} & \colorbox[rgb]{0.7643,0.9410,0.7138}{29.19\%} & \colorbox[rgb]{0.7090,0.9272,0.6467}{36.04\%} & \colorbox[rgb]{0.8075,0.9518,0.7663}{23.84\%} & \colorbox[rgb]{0.7285,0.9321,0.6703}{33.63\%} & \colorbox[rgb]{0.7782,0.9445,0.7307}{27.47\%} & \colorbox[rgb]{0.9296,0.9824,0.9145}{8.72\%} & \colorbox[rgb]{0.9832,0.9958,0.9796}{2.08\%} \\
% 59 & StarCoder                      & StarCoder                      & \colorbox[rgb]{0.7525,0.9381,0.6994}{30.66\%} & \colorbox[rgb]{0.6289,0.9071,0.5493}{45.97\%} & \colorbox[rgb]{0.7554,0.9388,0.7029}{30.30\%} & \colorbox[rgb]{0.8129,0.9532,0.7727}{23.18\%} & \colorbox[rgb]{0.9521,0.9880,0.9419}{5.93\%} & \colorbox[rgb]{0.9645,0.9911,0.9569}{4.40\%} & \colorbox[rgb]{0.8008,0.9502,0.7581}{24.67\%} & \colorbox[rgb]{0.7642,0.9410,0.7136}{29.21\%} & \colorbox[rgb]{0.6685,0.9171,0.5974}{41.06\%} & \colorbox[rgb]{0.7596,0.9398,0.7080}{29.78\%} & \colorbox[rgb]{0.7039,0.9259,0.6404}{36.68\%} & \colorbox[rgb]{0.8682,0.9670,0.8399}{16.33\%} & \colorbox[rgb]{0.8929,0.9732,0.8699}{13.27\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 60 & CodeGen2.5                     & CodeGen2.5-7B-Instruct         & \colorbox[rgb]{0.7613,0.9403,0.7101}{29.57\%} & \colorbox[rgb]{0.5934,0.8983,0.5063}{50.36\%} & \colorbox[rgb]{0.8218,0.9554,0.7836}{22.07\%} & \colorbox[rgb]{0.8365,0.9591,0.8015}{20.25\%} & \colorbox[rgb]{0.9462,0.9865,0.9346}{6.67\%} & \colorbox[rgb]{0.9963,0.9991,0.9955}{0.46\%} & \colorbox[rgb]{0.7678,0.9419,0.7180}{28.76\%} & \colorbox[rgb]{0.7904,0.9476,0.7455}{25.96\%} & \colorbox[rgb]{0.6956,0.9238,0.6304}{37.70\%} & \colorbox[rgb]{0.7920,0.9479,0.7474}{25.77\%} & \colorbox[rgb]{0.7388,0.9347,0.6828}{32.35\%} & \colorbox[rgb]{0.8001,0.9500,0.7573}{24.76\%} & \colorbox[rgb]{0.9068,0.9767,0.8869}{11.54\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 61 & InternLM                       & InternLM-20B                   & \colorbox[rgb]{0.7626,0.9406,0.7117}{29.41\%} & \colorbox[rgb]{0.6027,0.9006,0.5175}{49.21\%} & \colorbox[rgb]{0.7968,0.9492,0.7532}{25.17\%} & \colorbox[rgb]{0.8546,0.9636,0.8234}{18.01\%} & \colorbox[rgb]{0.9612,0.9903,0.9528}{4.81\%} & \colorbox[rgb]{0.9860,0.9965,0.9829}{1.74\%} & \colorbox[rgb]{0.7701,0.9425,0.7208}{28.48\%} & \colorbox[rgb]{0.8007,0.9501,0.7579}{24.69\%} & \colorbox[rgb]{0.7174,0.9293,0.6569}{35.00\%} & \colorbox[rgb]{0.7514,0.9378,0.6981}{30.79\%} & \colorbox[rgb]{0.7612,0.9402,0.7100}{29.58\%} & \colorbox[rgb]{0.7882,0.9470,0.7428}{26.23\%} & \colorbox[rgb]{0.8820,0.9705,0.8567}{14.62\%} & \colorbox[rgb]{0.6965,0.9240,0.6314}{37.60\%} \\
% 62 & DeepSeek Coder                 & deepseek-coder-5.7bmqa-base    & \colorbox[rgb]{0.7665,0.9416,0.7165}{28.92\%} & \colorbox[rgb]{0.6317,0.9078,0.5527}{45.62\%} & \colorbox[rgb]{0.7327,0.9331,0.6754}{33.11\%} & \colorbox[rgb]{0.9058,0.9764,0.8856}{11.67\%} & \colorbox[rgb]{0.9633,0.9908,0.9555}{4.54\%} & \colorbox[rgb]{0.9636,0.9909,0.9558}{4.51\%} & \colorbox[rgb]{0.7835,0.9458,0.7371}{26.82\%} & \colorbox[rgb]{0.7787,0.9446,0.7313}{27.41\%} & \colorbox[rgb]{0.6943,0.9235,0.6287}{37.87\%} & \colorbox[rgb]{0.8129,0.9532,0.7728}{23.17\%} & \colorbox[rgb]{0.7526,0.9381,0.6996}{30.64\%} & \colorbox[rgb]{0.7987,0.9496,0.7556}{24.93\%} & \colorbox[rgb]{0.9141,0.9785,0.8957}{10.64\%} & \colorbox[rgb]{0.8423,0.9605,0.8084}{19.54\%} \\
% 63 & ChatGLM                        & ChatGLM3-6B                    & \colorbox[rgb]{0.7721,0.9430,0.7232}{28.23\%} & \colorbox[rgb]{0.6571,0.9142,0.5835}{42.48\%} & \colorbox[rgb]{0.7831,0.9457,0.7366}{26.87\%} & \colorbox[rgb]{0.8322,0.9580,0.7963}{20.78\%} & \colorbox[rgb]{0.9464,0.9866,0.9349}{6.64\%} & \colorbox[rgb]{0.9514,0.9878,0.9410}{6.02\%} & \colorbox[rgb]{0.7532,0.9382,0.7003}{30.57\%} & \colorbox[rgb]{0.8240,0.9560,0.7863}{21.80\%} & \colorbox[rgb]{0.7603,0.9400,0.7089}{29.69\%} & \colorbox[rgb]{0.7429,0.9357,0.6877}{31.85\%} & \colorbox[rgb]{0.7665,0.9416,0.7165}{28.92\%} & \colorbox[rgb]{0.7721,0.9430,0.7232}{28.23\%} & \colorbox[rgb]{0.9334,0.9833,0.9191}{8.25\%} & \colorbox[rgb]{0.7819,0.9454,0.7352}{27.01\%} \\
% 64 & Baichuan2                      & Baichuan2-7B-Chat              & \colorbox[rgb]{0.7778,0.9444,0.7301}{27.53\%} & \colorbox[rgb]{0.6598,0.9149,0.5869}{42.14\%} & \colorbox[rgb]{0.7673,0.9418,0.7174}{28.83\%} & \colorbox[rgb]{0.8641,0.9660,0.8349}{16.84\%} & \colorbox[rgb]{0.9713,0.9928,0.9652}{3.55\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.7657,0.9414,0.7155}{29.02\%} & \colorbox[rgb]{0.7872,0.9468,0.7416}{26.36\%} & \colorbox[rgb]{0.7343,0.9335,0.6774}{32.91\%} & \colorbox[rgb]{0.8415,0.9603,0.8075}{19.63\%} & \colorbox[rgb]{0.7715,0.9428,0.7225}{28.30\%} & \colorbox[rgb]{0.7788,0.9447,0.7314}{27.40\%} & \colorbox[rgb]{0.9705,0.9926,0.9642}{3.65\%} & \colorbox[rgb]{0.5991,0.8997,0.5131}{49.66\%} \\
% 65 & Qwen                           & Qwen-1.8B-Chat                 & \colorbox[rgb]{0.7833,0.9458,0.7369}{26.84\%} & \colorbox[rgb]{0.6743,0.9185,0.6044}{40.35\%} & \colorbox[rgb]{0.7970,0.9492,0.7534}{25.15\%} & \colorbox[rgb]{0.8184,0.9546,0.7794}{22.50\%} & \colorbox[rgb]{0.9901,0.9975,0.9879}{1.23\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.7742,0.9435,0.7258}{27.97\%} & \colorbox[rgb]{0.7802,0.9450,0.7330}{27.23\%} & \colorbox[rgb]{0.7828,0.9456,0.7362}{26.91\%} & \colorbox[rgb]{0.8048,0.9512,0.7629}{24.18\%} & \colorbox[rgb]{0.7659,0.9414,0.7157}{29.00\%} & \colorbox[rgb]{0.7960,0.9490,0.7523}{25.27\%} & \colorbox[rgb]{0.9531,0.9883,0.9430}{5.81\%} & \colorbox[rgb]{0.8414,0.9603,0.8074}{19.65\%} \\
% 66 & DeepSeek MoE                   & deepseek-moe-16b-base          & \colorbox[rgb]{0.7849,0.9462,0.7387}{26.65\%} & \colorbox[rgb]{0.6635,0.9158,0.5914}{41.68\%} & \colorbox[rgb]{0.7440,0.9359,0.6891}{31.71\%} & \colorbox[rgb]{0.9009,0.9752,0.8797}{12.27\%} & \colorbox[rgb]{0.9660,0.9915,0.9587}{4.21\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.7732,0.9433,0.7246}{28.09\%} & \colorbox[rgb]{0.7926,0.9481,0.7481}{25.69\%} & \colorbox[rgb]{0.7485,0.9371,0.6946}{31.15\%} & \colorbox[rgb]{0.8413,0.9603,0.8073}{19.66\%} & \colorbox[rgb]{0.7758,0.9439,0.7277}{27.77\%} & \colorbox[rgb]{0.7811,0.9452,0.7342}{27.11\%} & \colorbox[rgb]{0.9566,0.9891,0.9473}{5.38\%} & \colorbox[rgb]{0.8203,0.9550,0.7818}{22.26\%} \\
% 67 & Baichuan2                      & Baichuan2-13B-Base             & \colorbox[rgb]{0.7875,0.9468,0.7420}{26.32\%} & \colorbox[rgb]{0.6528,0.9131,0.5783}{43.01\%} & \colorbox[rgb]{0.8266,0.9566,0.7894}{21.48\%} & \colorbox[rgb]{0.8638,0.9659,0.8346}{16.87\%} & \colorbox[rgb]{0.9478,0.9869,0.9366}{6.47\%} & \colorbox[rgb]{0.9598,0.9899,0.9512}{4.98\%} & \colorbox[rgb]{0.8187,0.9546,0.7798}{22.46\%} & \colorbox[rgb]{0.7857,0.9464,0.7398}{26.54\%} & \colorbox[rgb]{0.7434,0.9358,0.6883}{31.79\%} & \colorbox[rgb]{0.7931,0.9482,0.7487}{25.63\%} & \colorbox[rgb]{0.7574,0.9393,0.7054}{30.05\%} & \colorbox[rgb]{0.8689,0.9672,0.8408}{16.24\%} & \colorbox[rgb]{0.9255,0.9814,0.9095}{9.23\%} & \colorbox[rgb]{0.8909,0.9727,0.8674}{13.52\%} \\
% 68 & DeepSeek LLM                   & deepseek-llm-7b-base           & \colorbox[rgb]{0.7954,0.9488,0.7516}{25.34\%} & \colorbox[rgb]{0.7047,0.9261,0.6414}{36.58\%} & \colorbox[rgb]{0.7530,0.9382,0.7001}{30.59\%} & \colorbox[rgb]{0.8762,0.9690,0.8497}{15.33\%} & \colorbox[rgb]{0.9838,0.9959,0.9803}{2.01\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.8418,0.9604,0.8079}{19.59\%} & \colorbox[rgb]{0.7786,0.9446,0.7312}{27.42\%} & \colorbox[rgb]{0.7640,0.9410,0.7134}{29.23\%} & \colorbox[rgb]{0.7803,0.9450,0.7331}{27.22\%} & \colorbox[rgb]{0.7685,0.9421,0.7189}{28.67\%} & \colorbox[rgb]{0.8789,0.9697,0.8529}{15.00\%} & \colorbox[rgb]{0.9276,0.9819,0.9121}{8.97\%} & \colorbox[rgb]{0.7958,0.9489,0.7521}{25.29\%} \\
% 69 & Llama 2                        & Llama2-13B                     & \colorbox[rgb]{0.8022,0.9505,0.7598}{24.50\%} & \colorbox[rgb]{0.6925,0.9231,0.6266}{38.09\%} & \colorbox[rgb]{0.7923,0.9480,0.7477}{25.73\%} & \colorbox[rgb]{0.8789,0.9697,0.8529}{15.00\%} & \colorbox[rgb]{0.9477,0.9869,0.9365}{6.48\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8284,0.9571,0.7917}{21.25\%} & \colorbox[rgb]{0.7974,0.9493,0.7540}{25.09\%} & \colorbox[rgb]{0.7709,0.9427,0.7218}{28.38\%} & \colorbox[rgb]{0.8039,0.9509,0.7619}{24.29\%} & \colorbox[rgb]{0.7837,0.9459,0.7374}{26.79\%} & \colorbox[rgb]{0.8402,0.9600,0.8059}{19.80\%} & \colorbox[rgb]{0.9219,0.9804,0.9051}{9.68\%} & \colorbox[rgb]{0.9627,0.9907,0.9547}{4.62\%} \\
% 70 & Baichuan2                      & Baichuan2-7B-Base              & \colorbox[rgb]{0.8103,0.9525,0.7696}{23.50\%} & \colorbox[rgb]{0.7046,0.9261,0.6413}{36.59\%} & \colorbox[rgb]{0.8068,0.9517,0.7654}{23.93\%} & \colorbox[rgb]{0.8950,0.9737,0.8724}{13.01\%} & \colorbox[rgb]{0.9516,0.9879,0.9413}{5.99\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.8301,0.9575,0.7936}{21.05\%} & \colorbox[rgb]{0.8149,0.9537,0.7752}{22.93\%} & \colorbox[rgb]{0.7660,0.9415,0.7159}{28.98\%} & \colorbox[rgb]{0.8265,0.9566,0.7893}{21.49\%} & \colorbox[rgb]{0.7899,0.9474,0.7448}{26.03\%} & \colorbox[rgb]{0.8439,0.9610,0.8105}{19.33\%} & \colorbox[rgb]{0.9622,0.9905,0.9541}{4.68\%} & \colorbox[rgb]{0.9136,0.9784,0.8951}{10.70\%} \\
% 71 & DeepSeek Coder                 & deepseek-coder-1.3b-base       & \colorbox[rgb]{0.8129,0.9532,0.7728}{23.17\%} & \colorbox[rgb]{0.7008,0.9251,0.6367}{37.06\%} & \colorbox[rgb]{0.7841,0.9460,0.7378}{26.74\%} & \colorbox[rgb]{0.9352,0.9838,0.9213}{8.03\%} & \colorbox[rgb]{0.9771,0.9943,0.9722}{2.84\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.8704,0.9676,0.8426}{16.05\%} & \colorbox[rgb]{0.8310,0.9577,0.7948}{20.93\%} & \colorbox[rgb]{0.7242,0.9310,0.6651}{34.16\%} & \colorbox[rgb]{0.8008,0.9501,0.7580}{24.68\%} & \colorbox[rgb]{0.7819,0.9454,0.7351}{27.02\%} & \colorbox[rgb]{0.8837,0.9709,0.8588}{14.40\%} & \colorbox[rgb]{0.9622,0.9905,0.9541}{4.68\%} & \colorbox[rgb]{0.7988,0.9497,0.7557}{24.92\%} \\
% 72 & Qwen                           & Qwen-1.8B                      & \colorbox[rgb]{0.8134,0.9533,0.7733}{23.12\%} & \colorbox[rgb]{0.6948,0.9236,0.6293}{37.81\%} & \colorbox[rgb]{0.8471,0.9617,0.8143}{18.94\%} & \colorbox[rgb]{0.8867,0.9716,0.8624}{14.04\%} & \colorbox[rgb]{0.9701,0.9925,0.9637}{3.70\%} & \colorbox[rgb]{0.9440,0.9860,0.9320}{6.94\%} & \colorbox[rgb]{0.8218,0.9554,0.7836}{22.07\%} & \colorbox[rgb]{0.8008,0.9501,0.7580}{24.68\%} & \colorbox[rgb]{0.7877,0.9469,0.7422}{26.30\%} & \colorbox[rgb]{0.8511,0.9628,0.8192}{18.44\%} & \colorbox[rgb]{0.7925,0.9481,0.7480}{25.70\%} & \colorbox[rgb]{0.8515,0.9628,0.8196}{18.40\%} & \colorbox[rgb]{0.9700,0.9925,0.9635}{3.72\%} & \colorbox[rgb]{0.8039,0.9509,0.7619}{24.29\%} \\
% 73 & Mistral                        & Mistral-7B-v0.1                & \colorbox[rgb]{0.8166,0.9541,0.7773}{22.72\%} & \colorbox[rgb]{0.7186,0.9296,0.6582}{34.86\%} & \colorbox[rgb]{0.8143,0.9535,0.7745}{23.00\%} & \colorbox[rgb]{0.8722,0.9680,0.8448}{15.83\%} & \colorbox[rgb]{0.9491,0.9873,0.9382}{6.30\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8385,0.9596,0.8038}{20.01\%} & \colorbox[rgb]{0.7940,0.9484,0.7498}{25.52\%} & \colorbox[rgb]{0.8043,0.9510,0.7624}{24.24\%} & \colorbox[rgb]{0.8279,0.9569,0.7910}{21.32\%} & \colorbox[rgb]{0.7981,0.9495,0.7548}{25.01\%} & \colorbox[rgb]{0.8590,0.9647,0.8287}{17.47\%} & \colorbox[rgb]{0.9167,0.9792,0.8988}{10.32\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 74 & Llama 2                        & Llama2-7B                      & \colorbox[rgb]{0.8196,0.9549,0.7809}{22.35\%} & \colorbox[rgb]{0.6977,0.9244,0.6328}{37.45\%} & \colorbox[rgb]{0.8278,0.9569,0.7909}{21.33\%} & \colorbox[rgb]{0.9193,0.9798,0.9020}{10.00\%} & \colorbox[rgb]{0.9851,0.9963,0.9819}{1.85\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.8339,0.9584,0.7983}{20.57\%} & \colorbox[rgb]{0.8482,0.9620,0.8157}{18.80\%} & \colorbox[rgb]{0.7684,0.9420,0.7187}{28.69\%} & \colorbox[rgb]{0.8183,0.9545,0.7793}{22.51\%} & \colorbox[rgb]{0.7959,0.9489,0.7522}{25.28\%} & \colorbox[rgb]{0.8525,0.9631,0.8209}{18.27\%} & \colorbox[rgb]{0.9938,0.9984,0.9925}{0.77\%} & \colorbox[rgb]{0.8980,0.9745,0.8761}{12.64\%} \\
% 75 & 01.AI                          & Yi-34B                         & \colorbox[rgb]{0.8223,0.9555,0.7842}{22.01\%} & \colorbox[rgb]{0.7204,0.9300,0.6604}{34.64\%} & \colorbox[rgb]{0.7864,0.9466,0.7406}{26.46\%} & \colorbox[rgb]{0.9376,0.9844,0.9242}{7.73\%} & \colorbox[rgb]{0.9851,0.9963,0.9819}{1.85\%} & \colorbox[rgb]{0.9663,0.9916,0.9591}{4.17\%} & \colorbox[rgb]{0.8131,0.9532,0.7730}{23.15\%} & \colorbox[rgb]{0.8631,0.9657,0.8337}{16.96\%} & \colorbox[rgb]{0.7468,0.9367,0.6925}{31.36\%} & \colorbox[rgb]{0.8763,0.9691,0.8498}{15.32\%} & \colorbox[rgb]{0.8135,0.9533,0.7735}{23.10\%} & \colorbox[rgb]{0.8192,0.9548,0.7804}{22.40\%} & \colorbox[rgb]{0.9504,0.9876,0.9397}{6.15\%} & \colorbox[rgb]{0.9075,0.9769,0.8876}{11.46\%} \\
% 76 & davinci                        & davinci-002                    & \colorbox[rgb]{0.8284,0.9571,0.7917}{21.25\%} & \colorbox[rgb]{0.7283,0.9320,0.6700}{33.66\%} & \colorbox[rgb]{0.8445,0.9611,0.8112}{19.26\%} & \colorbox[rgb]{0.8901,0.9725,0.8666}{13.61\%} & \colorbox[rgb]{0.9575,0.9894,0.9483}{5.27\%} & \colorbox[rgb]{0.9701,0.9925,0.9637}{3.70\%} & \colorbox[rgb]{0.8785,0.9696,0.8524}{15.05\%} & \colorbox[rgb]{0.8415,0.9603,0.8075}{19.63\%} & \colorbox[rgb]{0.7550,0.9387,0.7024}{30.35\%} & \colorbox[rgb]{0.8167,0.9541,0.7774}{22.70\%} & \colorbox[rgb]{0.7948,0.9487,0.7508}{25.42\%} & \colorbox[rgb]{0.8921,0.9730,0.8690}{13.36\%} & \colorbox[rgb]{0.9789,0.9947,0.9744}{2.61\%} & \colorbox[rgb]{0.9650,0.9913,0.9575}{4.33\%} \\
% 77 & Mixtral                        & mixtral-8x7B                   & \colorbox[rgb]{0.8288,0.9572,0.7921}{21.21\%} & \colorbox[rgb]{0.7355,0.9338,0.6788}{32.76\%} & \colorbox[rgb]{0.8342,0.9585,0.7986}{20.54\%} & \colorbox[rgb]{0.8770,0.9692,0.8507}{15.23\%} & \colorbox[rgb]{0.9701,0.9925,0.9637}{3.70\%} & \colorbox[rgb]{0.9832,0.9958,0.9796}{2.08\%} & \colorbox[rgb]{0.8544,0.9636,0.8231}{18.04\%} & \colorbox[rgb]{0.8868,0.9717,0.8625}{14.02\%} & \colorbox[rgb]{0.7375,0.9343,0.6813}{32.51\%} & \colorbox[rgb]{0.8161,0.9540,0.7767}{22.78\%} & \colorbox[rgb]{0.8097,0.9524,0.7689}{23.57\%} & \colorbox[rgb]{0.8910,0.9727,0.8676}{13.50\%} & \colorbox[rgb]{0.9193,0.9798,0.9020}{10.00\%} & \colorbox[rgb]{0.8706,0.9676,0.8428}{16.03\%} \\
% 78 & Phi                            & Phi1.5                         & \colorbox[rgb]{0.8340,0.9585,0.7984}{20.56\%} & \colorbox[rgb]{0.7405,0.9351,0.6848}{32.15\%} & \colorbox[rgb]{0.8336,0.9584,0.7979}{20.61\%} & \colorbox[rgb]{0.8848,0.9712,0.8601}{14.27\%} & \colorbox[rgb]{0.9726,0.9931,0.9667}{3.40\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8301,0.9575,0.7937}{21.04\%} & \colorbox[rgb]{0.8155,0.9538,0.7759}{22.86\%} & \colorbox[rgb]{0.8293,0.9573,0.7926}{21.15\%} & \colorbox[rgb]{0.8746,0.9686,0.8477}{15.53\%} & \colorbox[rgb]{0.8238,0.9559,0.7860}{21.83\%} & \colorbox[rgb]{0.8240,0.9560,0.7863}{21.80\%} & \colorbox[rgb]{0.9845,0.9961,0.9812}{1.92\%} & \colorbox[rgb]{0.8872,0.9718,0.8630}{13.97\%} \\
% 79 & 01.AI                          & Yi-6B                          & \colorbox[rgb]{0.8391,0.9597,0.8046}{19.93\%} & \colorbox[rgb]{0.7430,0.9357,0.6878}{31.84\%} & \colorbox[rgb]{0.8473,0.9618,0.8146}{18.91\%} & \colorbox[rgb]{0.8940,0.9735,0.8713}{13.13\%} & \colorbox[rgb]{0.9920,0.9980,0.9903}{0.99\%} & \colorbox[rgb]{0.9776,0.9944,0.9727}{2.78\%} & \colorbox[rgb]{0.8890,0.9722,0.8652}{13.75\%} & \colorbox[rgb]{0.8085,0.9521,0.7674}{23.72\%} & \colorbox[rgb]{0.8100,0.9524,0.7692}{23.54\%} & \colorbox[rgb]{0.8356,0.9589,0.8003}{20.37\%} & \colorbox[rgb]{0.8109,0.9527,0.7704}{23.42\%} & \colorbox[rgb]{0.8823,0.9705,0.8571}{14.58\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.9633,0.9908,0.9555}{4.54\%} \\
% 80 & CodeGeeX                       & CodeGeeX2-6B                   & \colorbox[rgb]{0.8395,0.9598,0.8051}{19.88\%} & \colorbox[rgb]{0.7465,0.9366,0.6922}{31.40\%} & \colorbox[rgb]{0.8594,0.9648,0.8293}{17.41\%} & \colorbox[rgb]{0.8868,0.9717,0.8625}{14.02\%} & \colorbox[rgb]{0.9821,0.9955,0.9782}{2.22\%} & \colorbox[rgb]{0.9608,0.9902,0.9524}{4.86\%} & \colorbox[rgb]{0.8484,0.9621,0.8159}{18.78\%} & \colorbox[rgb]{0.8388,0.9597,0.8042}{19.97\%} & \colorbox[rgb]{0.7950,0.9487,0.7511}{25.39\%} & \colorbox[rgb]{0.8834,0.9708,0.8584}{14.44\%} & \colorbox[rgb]{0.8217,0.9554,0.7835}{22.08\%} & \colorbox[rgb]{0.8699,0.9675,0.8421}{16.11\%} & \colorbox[rgb]{0.9669,0.9917,0.9598}{4.10\%} & \colorbox[rgb]{0.9210,0.9802,0.9041}{9.78\%} \\
% 81 & CodeGen2                       & CodeGen2-16B                   & \colorbox[rgb]{0.8630,0.9657,0.8336}{16.97\%} & \colorbox[rgb]{0.7783,0.9445,0.7308}{27.46\%} & \colorbox[rgb]{0.8523,0.9630,0.8206}{18.30\%} & \colorbox[rgb]{0.9348,0.9837,0.9208}{8.08\%} & \colorbox[rgb]{0.9901,0.9975,0.9879}{1.23\%} & \colorbox[rgb]{0.9888,0.9972,0.9864}{1.39\%} & \colorbox[rgb]{0.8951,0.9737,0.8725}{13.00\%} & \colorbox[rgb]{0.8605,0.9651,0.8306}{17.28\%} & \colorbox[rgb]{0.8059,0.9514,0.7643}{24.04\%} & \colorbox[rgb]{0.8851,0.9713,0.8605}{14.23\%} & \colorbox[rgb]{0.8323,0.9580,0.7964}{20.77\%} & \colorbox[rgb]{0.9388,0.9847,0.9257}{7.58\%} & \colorbox[rgb]{0.9431,0.9858,0.9309}{7.05\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} \\
% 82 & Phi                            & Phi2                           & \colorbox[rgb]{0.8649,0.9662,0.8359}{16.74\%} & \colorbox[rgb]{0.7662,0.9415,0.7161}{28.96\%} & \colorbox[rgb]{0.8872,0.9718,0.8630}{13.97\%} & \colorbox[rgb]{0.9336,0.9834,0.9193}{8.23\%} & \colorbox[rgb]{0.9587,0.9897,0.9498}{5.12\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8591,0.9648,0.8289}{17.45\%} & \colorbox[rgb]{0.8830,0.9707,0.8579}{14.49\%} & \colorbox[rgb]{0.8614,0.9653,0.8317}{17.17\%} & \colorbox[rgb]{0.8524,0.9631,0.8208}{18.28\%} & \colorbox[rgb]{0.8497,0.9624,0.8174}{18.62\%} & \colorbox[rgb]{0.8924,0.9731,0.8693}{13.33\%} & \colorbox[rgb]{0.9860,0.9965,0.9830}{1.73\%} & \colorbox[rgb]{0.8532,0.9633,0.8218}{18.18\%} \\
% 83 & InternLM                       & InternLM-7B                    & \colorbox[rgb]{0.8687,0.9672,0.8406}{16.26\%} & \colorbox[rgb]{0.7968,0.9492,0.7532}{25.17\%} & \colorbox[rgb]{0.8842,0.9710,0.8594}{14.34\%} & \colorbox[rgb]{0.9123,0.9781,0.8935}{10.86\%} & \colorbox[rgb]{0.9791,0.9948,0.9746}{2.59\%} & \colorbox[rgb]{0.9495,0.9874,0.9387}{6.25\%} & \colorbox[rgb]{0.9315,0.9829,0.9169}{8.48\%} & \colorbox[rgb]{0.8632,0.9658,0.8338}{16.95\%} & \colorbox[rgb]{0.7567,0.9391,0.7045}{30.14\%} & \colorbox[rgb]{0.9135,0.9784,0.8950}{10.71\%} & \colorbox[rgb]{0.8370,0.9592,0.8021}{20.19\%} & \colorbox[rgb]{0.9605,0.9901,0.9521}{4.89\%} & \colorbox[rgb]{0.9845,0.9961,0.9812}{1.92\%} & \colorbox[rgb]{0.7998,0.9499,0.7569}{24.80\%} \\
% 84 & IEITYuan                       & Yuan2-51B-hf                   & \colorbox[rgb]{0.8769,0.9692,0.8505}{15.25\%} & \colorbox[rgb]{0.7933,0.9483,0.7489}{25.61\%} & \colorbox[rgb]{0.9015,0.9754,0.8804}{12.20\%} & \colorbox[rgb]{0.9511,0.9878,0.9406}{6.06\%} & \colorbox[rgb]{0.9776,0.9944,0.9727}{2.78\%} & \colorbox[rgb]{0.9328,0.9832,0.9183}{8.33\%} & \colorbox[rgb]{0.8372,0.9593,0.8024}{20.16\%} & \colorbox[rgb]{0.8678,0.9669,0.8395}{16.37\%} & \colorbox[rgb]{0.8758,0.9689,0.8492}{15.38\%} & \colorbox[rgb]{0.9616,0.9904,0.9533}{4.76\%} & \colorbox[rgb]{0.8782,0.9695,0.8521}{15.09\%} & \colorbox[rgb]{0.8641,0.9660,0.8350}{16.83\%} & \colorbox[rgb]{0.9845,0.9961,0.9812}{1.92\%} & \colorbox[rgb]{0.7614,0.9403,0.7103}{29.55\%} \\
% 85 & Phi                            & Phi1                           & \colorbox[rgb]{0.8847,0.9712,0.8600}{14.28\%} & \colorbox[rgb]{0.8322,0.9580,0.7963}{20.78\%} & \colorbox[rgb]{0.8609,0.9652,0.8311}{17.23\%} & \colorbox[rgb]{0.9348,0.9837,0.9208}{8.08\%} & \colorbox[rgb]{0.9526,0.9881,0.9425}{5.87\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.9333,0.9833,0.9190}{8.26\%} & \colorbox[rgb]{0.8472,0.9618,0.8144}{18.93\%} & \colorbox[rgb]{0.8540,0.9635,0.8226}{18.09\%} & \colorbox[rgb]{0.8958,0.9739,0.8734}{12.91\%} & \colorbox[rgb]{0.8544,0.9636,0.8231}{18.04\%} & \colorbox[rgb]{0.9731,0.9933,0.9674}{3.33\%} & \colorbox[rgb]{0.9897,0.9974,0.9875}{1.28\%} & \colorbox[rgb]{0.7849,0.9462,0.7387}{26.65\%} \\
% 86 & CodeGen                        & CodeGen-16B-multi              & \colorbox[rgb]{0.8900,0.9725,0.8665}{13.62\%} & \colorbox[rgb]{0.8322,0.9580,0.7962}{20.79\%} & \colorbox[rgb]{0.8935,0.9734,0.8707}{13.19\%} & \colorbox[rgb]{0.9123,0.9781,0.8935}{10.86\%} & \colorbox[rgb]{0.9771,0.9943,0.9722}{2.84\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.9083,0.9771,0.8886}{11.36\%} & \colorbox[rgb]{0.8555,0.9638,0.8245}{17.90\%} & \colorbox[rgb]{0.8914,0.9728,0.8681}{13.45\%} & \colorbox[rgb]{0.9077,0.9769,0.8879}{11.43\%} & \colorbox[rgb]{0.8673,0.9668,0.8388}{16.44\%} & \colorbox[rgb]{0.9443,0.9861,0.9324}{6.90\%} & \colorbox[rgb]{0.9751,0.9938,0.9698}{3.08\%} & \colorbox[rgb]{0.9292,0.9823,0.9140}{8.77\%} \\
% 87 & IEITYuan                       & Yuan2-102B-hf                  & \colorbox[rgb]{0.9154,0.9788,0.8973}{10.48\%} & \colorbox[rgb]{0.8532,0.9633,0.8218}{18.18\%} & \colorbox[rgb]{0.9373,0.9843,0.9238}{7.77\%} & \colorbox[rgb]{0.9449,0.9862,0.9331}{6.82\%} & \colorbox[rgb]{0.9851,0.9963,0.9819}{1.85\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8618,0.9654,0.8322}{17.12\%} & \colorbox[rgb]{0.9237,0.9809,0.9074}{9.45\%} & \colorbox[rgb]{0.9458,0.9864,0.9342}{6.71\%} & \colorbox[rgb]{0.9577,0.9894,0.9486}{5.24\%} & \colorbox[rgb]{0.9321,0.9830,0.9175}{8.41\%} & \colorbox[rgb]{0.8520,0.9630,0.8203}{18.33\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.8457,0.9614,0.8126}{19.11\%} \\
% 88 & IEITYuan                       & Yuan2-2B-hf                    & \colorbox[rgb]{0.9412,0.9853,0.9286}{7.28\%} & \colorbox[rgb]{0.9265,0.9816,0.9107}{9.11\%} & \colorbox[rgb]{0.9345,0.9836,0.9205}{8.11\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.9551,0.9888,0.9455}{5.56\%} & \colorbox[rgb]{0.9776,0.9944,0.9727}{2.78\%} & \colorbox[rgb]{0.9676,0.9919,0.9607}{4.01\%} & \colorbox[rgb]{0.9331,0.9833,0.9187}{8.29\%} & \colorbox[rgb]{0.9170,0.9792,0.8992}{10.28\%} & \colorbox[rgb]{0.9385,0.9846,0.9253}{7.62\%} & \colorbox[rgb]{0.9290,0.9822,0.9137}{8.80\%} & \colorbox[rgb]{0.9655,0.9914,0.9581}{4.27\%} & \colorbox[rgb]{1.0000,1.0000,1.0000}{0.00\%} & \colorbox[rgb]{0.9491,0.9873,0.9381}{6.31\%} \\


       

%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

